Towards a Better Understanding of Learning with Multiagent Teams

While it has long been recognized that a team of individual learning agents can be greater than the sum of its parts, recent work has shown that larger teams are not necessarily more effective than smaller ones. In this paper, we study why and under which conditions certain team structures promote effective learning for a population of individual learning agents. We show that, depending on the environment, some team structures help agents learn to specialize into specific roles, resulting in more favorable global results. However, large teams create credit assignment challenges that reduce coordination, leading to large teams performing poorly compared to smaller ones. We support our conclusions with both theoretical analysis and empirical results.

==> Submit/AAAI23-Submit/rebuttal_notes.tex <==

NOTE: Every line that starts with "(DTR) --> " is a thought that Dave has had in response to the above comment for the rebuttal.
"(KL) is Kate's comment.
"(TB) for Tim's comments




Reviewer #2
Questions


2. {Strengths and Weaknesses} 
This paper shows how teams can help agents identify reward-causing state-action pairs, but sub-optimal team structures can induce environments where agents are unable to learn. And comparisons between the impact of teams on learning and several commonly studied areas across RL research. 
The main issue of this work is about the scalability. It is not only about the number of agents, but the state space. The authors seem to ignore such potential issues while focusing on a small number of states. Some minor suggestions:

1) Below formula 1, when $R_i^t$ is represented, the state of the next time slice is represented in normal font, and the representation of the previous state and action is in bold font.

(DTR) --> I'm not sure what the reviewer means in pointing this out. This is intentional (because $s_i^{t+1}$ is not a joint state, and is explained below Formula 1 where they point it out.

(KL): Ignore it -- the reviewer said it was minor. Don't waste time or responding. Just thank them for their comments in general and move on.
(TB): Agree

2) Referring to Figure 1, which introduces two states, it is recommended to add a legend to assist understanding when introducing four states environment.

(DTR) --> A legend could be added, but this might be confusing in Figure 1. A diagram of 4-States could be included in the appendix.

(KL): Legend might be better since, if accepted, the appendix is not published.
(TB): Could just add the info to the caption? But it would be good to have it here?


3) In future work, it is recommended that the authors consider more multi-agent problems, increase comparative experiments, or extend research in partially observable environments.

(DTR) --> We intend to expand this work to the Neural MMO environment in future work; however, all three environments used in our evaluation (including the appendix) are already partially observable. Cleanup was specifically chosen because it is a popular environment shown to be challenging for RL agents to learn in and previous work often benchmarks against the setting when the entire population is cooperative. The main motivation of this paper is to show that choosing a fully cooperative population to be a benchmark is not always a good idea.

(KL): This is a fine response.
(TB): change "population to be a benchmark" to "basis for comparision"? or to
      choosing to benchmark against a fully cooperative population

3. {Questions for the Authors} Please carefully describe questions that you would like the authors to answer during the author feedback period. Think of the things where a response from the author may change your opinion, clarify a confusion or address a limitation. Please number your questions.
1. Howe would the authors justify the quality of the experimental results if the optimal ones are unknown?

(DTR) --> While we know the optimal result in 4-States and the IPD (appendix), Cleanup is more difficult due to the many stochastic environmental properties. In this scenario, we justify the quality of the results by comparing different sized teams together (showing how performance decreases with larger teams), and how $n=2$ and $n=4$ both achieve roughly the highest published mean population reward in the environment as shown in the cited papers (Radke, Larson, Brecht, 2022a,b).

(KL): OK
(TB): comparing different sized teams together -> 
      comparing different sized teams with each other
      If the paper doesn't already say this at some point maybe you can
      explictly state that these are the highest known results to date.

2. what is potential risks of increasing the number of states in the problem domains?

(DTR) --> The answer to this depends on if it is about ``joint" states or physical/individually observed states. 1) The joint state space is exponential in the number of agents, so the joint state space increases each time an agent is added. 2) If more waste states are added to 4-States, our results will be greater emphasized since agents on larger teams will have a higher probability of choosing states with reward of 0 instead of the optimal solution. In the IPD, the state space is directly dependent on $N$, and Cleanup is a bounded environment commonly used across different work. Spatially expanding Cleanup does not change our results. Given Cleanup's reward distribution, we have shown that agents on larger teams fail to learn meaningful policies. This is independent of the size of the environment.

OR:

(DTR) --> We do not increase the number of physical states in our analysis because we focus on relating the states they learn from conceptually. That is, we are interested in how the information signal changes across an environment as their team size increases, independent of the number of states. Increasing the number of states may not impact our results as much as changing the underlying reward function of an environment.

(KL): I like this response -- it is getting to the heart of the comment. The first is too specific.
(TB): Agree

3. how do you measure the policy or rewards through information entropy?

(DTR) --> Information entropy is a way to measure the information from the environments agents use to learn from. Information is gained though rewards, not as a way to measure rewards. If a policy has converged to some non-stochastic behavior, this means they have used the information in the environment to do so. Our work shows that information entropy converges to 0 as $n$ increases, and agents become more stochastic.

(KL): good. This comment is showing a lack of understanding on the side of the reviewer. Your comment hopefully clarifies things for them.
(TB): Agree

4. Will the rewards be increased in a monotonic way when the number of agents increase?

(DTR) --> No, the main finding of this paper is to show that reward can eventually decrease as the size of a team increases because agents have more difficulty learning effective policies. This is shown in our experiments in the text and appendix as $n$ increases.

(KL): Good.
(TB): Agree

************************************************************
************************************************************
************************************************************



Reviewer #5
Questions


2. {Strengths and Weaknesses} 

The research could improve the development of multiagent teams and it’s helpful for researchers to choose better team network structures.

3. {Questions for the Authors} 
My detailed comments are as follows:

1. The author didn’t provide enough explaination about the role specialization mentioned in the Abstract and Cleanup Gridworld Game Results. It is essential to explain how it relates to the main theme of the study, which is how team structures shape the learning processes and environments for individual agents.

(DTR) --> We will elaborate on the specific types of roles in each environment in the camera ready version. We will also add more explanation into the results about the spatial component of role specialization to further emphasize Figure 5.

2. The author’s description of credit assignment is not clear or complete, especially the realted work or background information about credit assignment.

(DTR) --> We plan to add more general detail on credit assignment in the related work/background, and narrow the scope in the later sections on information sparsity where we discuss it more relating to our work.

(KL): Can you expand on this point -- to show the reviewer what you might include in the paper -- ie what you will highlight?
(TB): Good idea.


3. The author didn’t provide enought detail about how teams guide agents to identify reward-causing state-action pairs in the section: Identifying Valuable State-Action Pairs. The author described the definition of “reward-causing state-action pairs” and the example environment, and pointed that increasing team size will increase the team-based reward. However, the identification of valuable state-action pairs is not mentioned here.

(DTR) --> The main distinction in this section is not that increasing team size will simply increase team-based reward, but rather that increasing team size increases the probability of the team-based reward being non-zero at reward-causing state-action pairs. This increases the reward signal at these state-action pairs compared to situations when there are no teams, helping agents learn to execute those state-action pairs more regularly.

(KL): good.
(TB): agree

4. The author ‘s analysis about the risk of sub-optimal team structure should be in a separate section, because this part is analyzed through reward-causing state-action pairs identification and credit assignment challenges.

(DTR) --> It is in a separate section, but maybe they didn't realize this because they arent numbered?

(KL): Technically it is in a separate subsection... You can say that you could certainly make it its own section, though space constraints may mean you need to keep it as a subsection.
(TB): I might point out that it is in a separate subsection but because the
latex template doesn't number it as such it might not appear so?




************************************************************
************************************************************
************************************************************


Reviewer #6
Questions


2. {Strengths and Weaknesses} 
Strengths:

-Aiming to get insights on how team structure influences the individual learning process is an interesting question. 
-Providing theories on team structure and its effect on reward mechanism 
-Justifying the theories with the empirical results.

Weakness:

-Some empirical results are not so convincing to justify the presented theories (e.g. cleaning up ). The empirical data could be extended and investigated more elaborately the effect of varying values for n. For instance, for the first problem we can observe the results for n1,2,4,8,16 but for the second problem we can only see n=4 and n=6 comparisons.

(DTR) --> We only compared $n=4$ and $n=6$ to conserve space and because the reasoning for a decrease in reward (duplication of roles) is consistent with teams larger than 4.

(KL): OK. 
(TB): agree

-Team structure seems to be measured by the number of agents in a team. Their cooperativeness level and conflict level within the team are not considered yet. 

(DTR) --> We assume teams to be fully cooperative (fully share rewards) since past work often benchmarks solutions with this scenario. The motivation of this paper is to provide an explanation as to why a fully cooperative population may actually achieve worse performance.

(KL): OK
(TB): agree - Dave: it feels like the word benchmark being used a bit awkwardly.
Isn't the benchmark actually Cleanup (i.e., the software being used
to evaluate different systems)
but the fully cooperative population is the basis for comparison
(or state-of-the-art approach/configuration/solution?).

-There is no explicit insight about the desired number of teams for the optimal learning updates. In the experiments, it can be observed for the first problem, a team size of two yields a good performance but depending on the problem and size of the problem it may vary. Maybe, the reviewer overlooked it but could not see any guidance on the optimal choice of team size. 

(DTR) --> We discuss that it does depend on the number of reward-causing state-action pairs; however, this does vary greatly depending on the environment. We have shown that teams increase the ability to identify reward-causing state-action pairs until they induce $(\epsilon, \mu)$-information sparsity. Thus, one answer could be a team of multiple agents that does not induce $(\epsilon, \mu)$-information sparsity.

(KL): I would also add a sentence saying that in the final version you will emphasize this point and discuss it further.
(TB): I like what Kate suggests

-Limited novelty and contribution


3. {Questions for the Authors}
Have you investigated how agents perform for the cases when n= 8 and n=16 for the cleanup problem ? Were they worse than n=4?

(DTR) --> We did not experiment with teams greater than size 7 since all previous work uses up to 5 (and occasionally 6) agents. We could explore $n=8$ and $n=16$ in future work, though our results show a monotonic trend in reward and $\pi_i$-entropy with teams larger than $n=4$.

(TB): change to "since previous work use a maximum of 6 agents".
Don't say all b/c there might be something you've missed.
Maybe "We could explore ....,
however our results show ...



************************************************************
************************************************************
************************************************************



Reviewer #7
Questions

2. {Strengths and Weaknesses}
Strengths: 

+ This paper is well written and easy to understand.
+ Two new environments in reinforcement learning have been proposed in this paper.

Weaknesses:

+ When dealing with team member rewards, it is not novel enough to just distribute the rewards obtained by each agent equally to each member. The experimental environment provided in this paper is relatively simple, and is specially designed for the problems in this paper, and the generality is not enough. 

(DTR) --> The contributions of this work are not a novel way to distribute rewards, but to generally understand how teams impact the learning process of agents across three different learning environments and algorithms (IPD in appendix).

(KL): Say something like "We will emphasize this point further in our final version."
(TB): You might also point out that you are simply using the approach used
      in previous work - for a fair comparison.

+ In Lemma 1 derivation of the article, the proof is based on the central limit theorem, but the agents used in the experiment is very few. 

(DTR) --> The theory provides an understanding of how reward variance is shaped by the size of a team (converges to 0); however, we do not need infinite agents for RL to fail in practice. Our empirical evaluation is to confirm that increasing the size of a team reduces the ability for agents to learn, despite many recent works using this setting as a benchmark.

(KL): good
(TB): 
"recent works" -> recent research
"benchmark" -> basis for comparison (or something like state-of-the-art approaches)
Somewhere earlier you need to make it very clear the settings/conditions
under which the previous best results have been obtained
in this environment. And that you obtain better results (if that's actually the case).

+ In Figure 5 and Figure 6, there are six methods, why each subfigure only plots the performance of four methods, and the four methods are different across subfigures?

(DTR) --> (Assuming it is for Figure 5 as we do not have a Figure 6 in the main text) This plot shows the policies 3 individual agents learn when $n=4$ and $n=6$. Yes, there are two agents when $n=6$ that perform the same policy and have duplicate (and redundant) roles. The reason for this plot is to show how agents converge to the same behavior when team size grows as a result of sub-optimal team size and reduced information from the environment.

(TB): The reason for -> The purpose of 

+ For Theorem 1: There exists an environment where increasing team size increases the probability of an agent receiving a reward for executing any reward-causing state-action pair that is greater than if they were not in a team. The experimental results only work best when there are two agents, which cannot explain the theorem. The experiment is not very convincing.

(DTR) --> Theorem 1 explains how increasing the size of a team increases the probability of gaining a non-zero reward for reward-causing state-action pairs (i.e., teams can learn about valuable areas of the state space to generate more reward than single agents). However, Theorem 2 explains that too large of teams will hinder performance. This is indeed exactly what each of our experiments shows, across different RL algorithms and environments.

(TB): that too large of teams -> teams that are too large
probably remove "indeed" because with it for some reason it seems
a bit aggressive :-)

3. {Questions for the Authors} Please carefully describe questions that you would like the authors to answer during the author feedback period. Think of the things where a response from the author may change your opinion, clarify a confusion or address a limitation. Please number your questions.

Hope author can provide the experimental results in a more valuable environment can be provided, such as smac or google football. It can also support the theory proposed in the article.

(DTR) --> SMAC and Google Football have defined group sizes in past work or upper bounds on the number of agents (on a football team). We intend to expand future work to Neural MMO, since the number of agents in that environment can expand to many agents.

(KL): good.
(TB): I'm not sure about "in past work". Is that relevant? Just
because it was done one way in the past, does that mean you have to
do it too? Will the reviewer understand clearly why it wouldn't make
sense to use these environments from your description?
Maybe "We intend to" --> "However, we intend to" -> "Instead, we intend to.

expand future work to ...
in future work we intend to study Neural MMO, ...

to many agents -> to a sufficiently large number of agents.






==> Submit/AAAI23-Submit/rebuttals.tex <==
To all: Thank you all for your comments and your time reviewing this work. I will address the points you have made individually below.

R2:
2.2) We will add a legend to Figure 1 in the final submission to clarify the changes to the environment for 4-States.

2.3) We intend to expand this work to the Neural MMO environment in future work, however all three environments used in our evaluation (IPD in appendix) are partially observable. Cleanup is a popular environment challenging for RL agents and a cooperative population is typically used as a basis for comparison. We show how assuming a fully cooperative population achieves the best performance is not a good idea in practice.

3.1) While we know the optimal result in 4-States and the IPD (appendix), Cleanup is more difficult due to the stochastic environment. We justify the quality of these results by comparing different sized teams with each other, and how n=2 or 4 achieve the highest published mean population reward (in Radke, Larson, Brecht, 2022a,b).

3.2) We dont increase the number of physical states because we focus on relating the states agents learn from conceptually. We are interested in how information changes across an environment as team size increases, independent of the number of states. Increasing states would have less effect than changing rewards.

3.3) Information entropy measures the information from the environment agents learn from. Information is gained though rewards, not to measure rewards. If an agent has non-stochastic behavior, they used the information in the environment to do so. Our work shows that information entropy converges to 0 as n increases.

3.4) No, the main finding of this paper is to show that reward can eventually decrease as the size of a team increases because agents have more difficulty learning effective policies. This is confirmed in our experiments.

R5:
3.1) We will elaborate on specific roles in each environment and add detail into the results about the spatial component of role specialization to emphasize Figure 5.

3.2) We will add more detail on credit assignment in the related work/background section about identifying the impacts of actions on the feedback signal. In later sections, we will narrow the scope about information sparsity in relation to our work.

3.3) The main distinction in this section is that increasing team size will increase the probability of the team-based reward being non-zero at reward-causing state-action pairs, not that this reward is strictly increasing. This increases the reward signal at state-action pairs compared to no teams, helping agents learn to execute those pairs more regularly.

3.4) We will make the analysis of sub-optimal team structure its own section in the final version.

R6:
2.1) We only compared n=4 and 6 to conserve space and because we observe duplication of roles in all teams larger than 4.

2.2) We assume teams to be fully cooperative (fully share rewards) since past work often uses this scenario as a basis of comparison. The motivation of this paper is to provide an explanation as to why a fully cooperative population may actually achieve worse performance.

2.3) We discuss that it does depend on the number of reward-causing state-action pairs; however, this does vary greatly depending on the environment. We have shown that teams increase the ability to identify reward-causing state-action pairs until they induce (eps, mu)-sparsity. One answer is a larger team that does not induce (eps, mu)-sparsity. We will emphasize this in the final version.

3.1) We did not experiment with teams greater than 7 since previous work uses a maximum of 6 agents. We could explore n>7 in future work, however our results show monotonic trends in reward and \pi_i-entropy when n>4.

R7:
2.1) The contributions of our work are not a novel way to distribute rewards, but to generally understand how teams impact the learning process of agents across three different learning environments and algorithms (IPD in appendix).

2.2) The theory provides an understanding of how reward variance is shaped by the size of a team (converges to 0); however, we do not need infinite agents for RL to fail in practice. Our empirical evaluation confirms this.

2.3) Fig 5 shows policies of 3 agents in each setup. The purpose of this figure is to show how agents learn redundant policies when n=6 due to reduced information.

2.3) Thm 1 shows increasing team size increases the probability of gaining a non-zero reward for reward-causing state-action pairs. Thm 2 shows too large of teams will hinder performance, which is exactly what each of our experiments show, across different RL algorithms and environments.

3.1) SMAC and Google Football have upper bounds on the number of agents (i.e., 11 agents on a football team). Instead, we intend to expand future work to Neural MMO since the number of agents in that environment can expand to a large number of agents.

==> Submit/AAAI23-Submit/reviews.tex <==


Reviewer #2
Questions

1. {Summary} Please briefly summarize the main claims/contributions of the paper in your own words. (Please do not include your evaluation of the paper here).
This work provides insight into why teams can assist agents in identifying valuable areas of the state space depending on the population’s team structure.
2. {Strengths and Weaknesses} Please provide a thorough assessment of the strengths and weaknesses of the paper, touching on each of the following dimensions: novelty, quality, clarity, and significance.
This paper shows how teams can help agents identify reward-causing state-action pairs, but sub-optimal team structures can induce environments where agents are unable to learn. And comparisons between the impact of teams on learning and several commonly studied areas across RL research. 
The main issue of this work is about the scalability. It is not only about the number of agents, but the state space. The authors seem to ignore such potential issues while focusing on a small number of states. Some minor suggestions:

1) Below formula 1, when $R_i^t$ is represented, the state of the next time slice is represented in normal font, and the representation of the previous state and action is in bold font.

2) Referring to Figure 1, which introduces two states, it is recommended to add a legend to assist understanding when introducing four states environment.

3) In future work, it is recommended that the authors consider more multi-agent problems, increase comparative experiments, or extend research in partially observable environments.
3. {Questions for the Authors} Please carefully describe questions that you would like the authors to answer during the author feedback period. Think of the things where a response from the author may change your opinion, clarify a confusion or address a limitation. Please number your questions.
1. Howe would the authors justify the quality of the experimental results if the optimal ones are unknown?

2. what is potential risks of increasing the number of states in the problem domains?

3. how do you measure the policy or rewards through information entropy?

4. Will the rewards be increased in a monotonic way when the number of agents increase?
4. {Evaluation: Novelty} How novel are the concepts, problems addressed, or methods introduced in the paper?
Fair: The paper contributes some new ideas or represents incremental advances.
5. {Evaluation: Quality} Is the paper technically sound?
Fair: The paper has minor technical flaws. For example, the proof of a theorem has some fixable errors or the experimental evaluation is weak.
6. {Evaluation: Significance} How do you rate the likely impact of the paper on the AI research community?
Fair: The paper is likely to have modest impact within a subfield of AI.
7. {Evaluation: Clarity} Is the paper well-organized and clearly written?
Fair: The paper is somewhat clear, but some important details are missing or unclear.
8. (Evaluation: Reproducibility) Are the results (e.g., theorems, experimental results) in the paper easily reproducible? (It may help to consult the paper’s reproducibility checklist.)checklist.)
Fair: key resources (e.g., proofs, code, data) are unavailable and/or some key details (e.g., proof sketches, experimental setup) are unavailable which make it difficult to reproduce the main results.
9. {Evaluation: Resources} If applicable, how would you rate the new resources (code, data sets) the paper contributes? (It might help to consult the paper’s reproducibility checklist)
Not applicable: For instance, the primary contributions of the paper are theoretical.
10. {Evaluation: Ethical considerations} Does the paper adequately address the applicable ethical considerations, e.g., responsible data collection and use (e.g., informed consent, privacy), possible societal harm (e.g., exacerbating injustice or discrimination due to algorithmic bias), etc.?
Not Applicable: The paper does not have any ethical considerations to address.
11. (OVERALL EVALUATION) Please provide your overall evaluation of the paper, carefully weighing the reasons to accept and the reasons to reject the paper.
Borderline reject: Technically solid paper where reasons to reject, e.g., poor novelty, outweigh reasons to accept, e.g. good quality. Please use sparingly.
13. (CONFIDENCE) How confident are you in your evaluation?
Somewhat confident, but there's a chance I missed some aspects. I did not carefully check some of the details, e.g., novelty, proof of a theorem, experimental design, or statistical validity of conclusions.
14. (EXPERTISE) How well does this paper align with your expertise?
Knowledgeable: This paper has some overlap with my current work. My recent work was focused on closely related topics and I am knowledgeable about most of the topics covered by the paper.


************************************************************
************************************************************
************************************************************



Reviewer #5
Questions

1. {Summary} Please briefly summarize the main claims/contributions of the paper in your own words. (Please do not include your evaluation of the paper here).
This paper examines how team structures can change how agents experience the underlying environments in various ways, thus having ramifications on agents’ learning processes. Valuable state-action pairs identifying and teams impact on credit assignment are two main research directions in this paper.
2. {Strengths and Weaknesses} Please provide a thorough assessment of the strengths and weaknesses of the paper, touching on each of the following dimensions: novelty, quality, clarity, and significance.
The research could improve the development of multiagent teams and it’s helpful for researchers to choose better team network structures.
3. {Questions for the Authors} Please carefully describe questions that you would like the authors to answer during the author feedback period. Think of the things where a response from the author may change your opinion, clarify a confusion or address a limitation. Please number your questions.
My detailed comments are as follows:

1. The author didn’t provide enough explaination about the role specialization mentioned in the Abstract and Cleanup Gridworld Game Results. It is essential to explain how it relates to the main theme of the study, which is how team structures shape the learning processes and environments for individual agents.

2. The author’s description of credit assignment is not clear or complete, especially the realted work or background information about credit assignment.

3. The author didn’t provide enought detail about how teams guide agents to identify reward-causing state-action pairs in the section: Identifying Valuable State-Action Pairs. The author described the definition of “reward-causing state-action pairs” and the example environment, and pointed that increasing team size will increase the team-based reward. However, the identification of valuable state-action pairs is not mentioned here.

4. The author ‘s analysis about the risk of sub-optimal team structure should be in a separate section, because this part is analyzed through reward-causing state-action pairs identification and credit assignment challenges.
4. {Evaluation: Novelty} How novel are the concepts, problems addressed, or methods introduced in the paper?
Good: The paper makes non-trivial advances over the current state-of-the-art.
5. {Evaluation: Quality} Is the paper technically sound?
Good: The paper appears to be technically sound. The proofs, if applicable, appear to be correct, but I have not carefully checked the details. The experimental evaluation, if applicable, is adequate, and the results convincingly support the main claims.
6. {Evaluation: Significance} How do you rate the likely impact of the paper on the AI research community?
Good: The paper is likely to have high impact within a subfield of AI OR modest impact across more than one subfield of AI.
7. {Evaluation: Clarity} Is the paper well-organized and clearly written?
Good: The paper is well organized but the presentation has minor details that could be improved.
8. (Evaluation: Reproducibility) Are the results (e.g., theorems, experimental results) in the paper easily reproducible? (It may help to consult the paper’s reproducibility checklist.)checklist.)
Good: key resources (e.g., proofs, code, data) are available and sufficient details (e.g., proofs, experimental setup) are described such that an expert should be able to reproduce the main results.
9. {Evaluation: Resources} If applicable, how would you rate the new resources (code, data sets) the paper contributes? (It might help to consult the paper’s reproducibility checklist)
Good: The shared resources are likely to be very useful to other AI researchers.
10. {Evaluation: Ethical considerations} Does the paper adequately address the applicable ethical considerations, e.g., responsible data collection and use (e.g., informed consent, privacy), possible societal harm (e.g., exacerbating injustice or discrimination due to algorithmic bias), etc.?
Good: The paper adequately addresses most, but not all, of the applicable ethical considerations.
11. (OVERALL EVALUATION) Please provide your overall evaluation of the paper, carefully weighing the reasons to accept and the reasons to reject the paper.
Accept: Technically solid paper, with high impact on at least one sub-area of AI or modest-to-high impact on more than one area of AI, with good to excellent quality, reproducibility, and if applicable, resources, and no unaddressed ethical considerations. Top 60% of accepted papers.
13. (CONFIDENCE) How confident are you in your evaluation?
Quite confident. I tried to check the important points carefully. It is unlikely, though conceivable, that I missed some aspects that could otherwise have impacted my evaluation.
14. (EXPERTISE) How well does this paper align with your expertise?
Very Knowledgeable: This paper significantly overlaps with my current work and I am very knowledgeable about most of the topics covered by the paper.



************************************************************
************************************************************
************************************************************


Reviewer #6
Questions

1. {Summary} Please briefly summarize the main claims/contributions of the paper in your own words. (Please do not include your evaluation of the paper here).
This paper studies the effect of team size (i.e., team shape) on learning of individual agents. The theories presented in this study are (1)increasing the team size increases the probability of receiving greater reward and (2) information converges to zero when the size of the team increases its limit. An empirical study is conducted to justify the proposed theories.
2. {Strengths and Weaknesses} Please provide a thorough assessment of the strengths and weaknesses of the paper, touching on each of the following dimensions: novelty, quality, clarity, and significance.
Strengths:

-Aiming to get insights on how team structure influences the individual learning process is an interesting question. 
-Providing theories on team structure and its effect on reward mechanism 
-Justifying the theories with the empirical results.

Weakness:

-Some empirical results are not so convincing to justify the presented theories (e.g. cleaning up ). The empirical data could be extended and investigated more elaborately the effect of varying values for n. For instance, for the first problem we can observe the results for n1,2,4,8,16 but for the second problem we can only see n=4 and n=6 comparisons. 

-Team structure seems to be measured by the number of agents in a team. Their cooperativeness level and conflict level within the team are not considered yet. 
-There is no explicit insight about the desired number of teams for the optimal learning updates. In the experiments, it can be observed for the first problem, team size of two yields a good performance but depending on the problem and size of the problem it may vary. Maybe, the reviewer overlooked it but could not see any guidance on the optimal choice of team size. 
-Limited novelty and contribution
3. {Questions for the Authors} Please carefully describe questions that you would like the authors to answer during the author feedback period. Think of the things where a response from the author may change your opinion, clarify a confusion or address a limitation. Please number your questions.
Have you investigated how agents perform for the cases when n= 8 and n=16 for the cleanup problem ? Were they worse than n=4?
4. {Evaluation: Novelty} How novel are the concepts, problems addressed, or methods introduced in the paper?
Fair: The paper contributes some new ideas or represents incremental advances.
5. {Evaluation: Quality} Is the paper technically sound?
Good: The paper appears to be technically sound. The proofs, if applicable, appear to be correct, but I have not carefully checked the details. The experimental evaluation, if applicable, is adequate, and the results convincingly support the main claims.
6. {Evaluation: Significance} How do you rate the likely impact of the paper on the AI research community?
Fair: The paper is likely to have modest impact within a subfield of AI.
7. {Evaluation: Clarity} Is the paper well-organized and clearly written?
Fair: The paper is somewhat clear, but some important details are missing or unclear.
8. (Evaluation: Reproducibility) Are the results (e.g., theorems, experimental results) in the paper easily reproducible? (It may help to consult the paper’s reproducibility checklist.)checklist.)
Fair: key resources (e.g., proofs, code, data) are unavailable and/or some key details (e.g., proof sketches, experimental setup) are unavailable which make it difficult to reproduce the main results.
9. {Evaluation: Resources} If applicable, how would you rate the new resources (code, data sets) the paper contributes? (It might help to consult the paper’s reproducibility checklist)
Not applicable: For instance, the primary contributions of the paper are theoretical.
10. {Evaluation: Ethical considerations} Does the paper adequately address the applicable ethical considerations, e.g., responsible data collection and use (e.g., informed consent, privacy), possible societal harm (e.g., exacerbating injustice or discrimination due to algorithmic bias), etc.?
Not Applicable: The paper does not have any ethical considerations to address.
11. (OVERALL EVALUATION) Please provide your overall evaluation of the paper, carefully weighing the reasons to accept and the reasons to reject the paper.
Borderline reject: Technically solid paper where reasons to reject, e.g., poor novelty, outweigh reasons to accept, e.g. good quality. Please use sparingly.
13. (CONFIDENCE) How confident are you in your evaluation?
Somewhat confident, but there's a chance I missed some aspects. I did not carefully check some of the details, e.g., novelty, proof of a theorem, experimental design, or statistical validity of conclusions.
14. (EXPERTISE) How well does this paper align with your expertise?
Somewhat Knowledgeable: This paper has little overlap with my current work. I am somewhat knowledgeable about some of the topics covered by the paper.


************************************************************
************************************************************
************************************************************



Reviewer #7
Questions

1. {Summary} Please briefly summarize the main claims/contributions of the paper in your own words. (Please do not include your evaluation of the paper here).
Presents how teams can assist agent training in a multi-agent environment. Some related theorems are proved, showing that learning with teams can gain more information from the environment.
2. {Strengths and Weaknesses} Please provide a thorough assessment of the strengths and weaknesses of the paper, touching on each of the following dimensions: novelty, quality, clarity, and significance.
Strengths: 

+ This paper is well written and easy to understand.
+ Two new environments in reinforcement learning have been proposed in this paper.



Weaknesses:

+ When dealing with team member rewards, it is not novel enough to just distribute the rewards obtained by each agent equally to each member. The experimental environment provided in this paper is relatively simple, and is specially designed for the problems in this paper, and the generality is not enough. 
+ In Lemma 1 derivation of the article, the proof is based on the central limit theorem, but the agents used in the experiment is very few. 
+ In Figure 5 and Figure 6, there are six methods, why each subfigure only plots the performance of four methods, and the four methods are different across subfigures?
+ For Theorem 1: There exists an environment where increasing team size increases the probability of an agent receiving a reward for executing any reward-causing state-action pair that is greater than if they were not in a team. The experimental results only work best when there are two agents, which cannot explain the theorem. The experiment is not very convincing.
3. {Questions for the Authors} Please carefully describe questions that you would like the authors to answer during the author feedback period. Think of the things where a response from the author may change your opinion, clarify a confusion or address a limitation. Please number your questions.
Hope author can provide the experimental results in a more valuable environment can be provided, such as smac or google football. It can also support the theory proposed in the article.
4. {Evaluation: Novelty} How novel are the concepts, problems addressed, or methods introduced in the paper?
Fair: The paper contributes some new ideas or represents incremental advances.
5. {Evaluation: Quality} Is the paper technically sound?
Fair: The paper has minor technical flaws. For example, the proof of a theorem has some fixable errors or the experimental evaluation is weak.
6. {Evaluation: Significance} How do you rate the likely impact of the paper on the AI research community?
Fair: The paper is likely to have modest impact within a subfield of AI.
7. {Evaluation: Clarity} Is the paper well-organized and clearly written?
Fair: The paper is somewhat clear, but some important details are missing or unclear.
8. (Evaluation: Reproducibility) Are the results (e.g., theorems, experimental results) in the paper easily reproducible? (It may help to consult the paper’s reproducibility checklist.)checklist.)
Poor: key details (e.g., proof sketches, experimental setup) are incomplete/unclear, or key resources (e.g., proofs, code, data) are unavailable.
9. {Evaluation: Resources} If applicable, how would you rate the new resources (code, data sets) the paper contributes? (It might help to consult the paper’s reproducibility checklist)
Not applicable: For instance, the primary contributions of the paper are theoretical.
10. {Evaluation: Ethical considerations} Does the paper adequately address the applicable ethical considerations, e.g., responsible data collection and use (e.g., informed consent, privacy), possible societal harm (e.g., exacerbating injustice or discrimination due to algorithmic bias), etc.?
Fair: The paper addresses some applicable ethical considerations but fails to address some important ones.
11. (OVERALL EVALUATION) Please provide your overall evaluation of the paper, carefully weighing the reasons to accept and the reasons to reject the paper.
Reject: For instance, a paper with poor quality, inadequate reproducibility, incompletely addressed ethical considerations.
13. (CONFIDENCE) How confident are you in your evaluation?
Quite confident. I tried to check the important points carefully. It is unlikely, though conceivable, that I missed some aspects that could otherwise have impacted my evaluation.
14. (EXPERTISE) How well does this paper align with your expertise?
Very Knowledgeable: This paper significantly overlaps with my current work and I am very knowledgeable about most of the topics covered by the paper.

==> Submit/IJCAI23-Submit/rebuttals.tex <==






Reviewer #1 - Weak Accept (6)

NO QUESTIONS

Reviewer #2 - Accept (7)

There is a related work [1], which also studies in benefits of teams. As [1] works on the similar topic to this paper, it is encouraged to have more discussion with [1].

References
[1] Radke, D., Larson, K., & Brecht, T. Exploring the Benefits of Teams in Multiagent Learning. IJCAI, 2022.


(DTR) --> Thanks for pointing this out. We do use this paper as motivation for our work; however, we primarily reference this paper's follow up work when discussing how sub-optimal team size can be bad. We will expand our discussion related to this paper in the camera ready version.

Reviewer #3 - Reject (4)
Questions

1. Summary
This paper theoretically proves that there exists an optimal number of agents for MARL training under a certain environment assumption, where 
(1) there are no communication with nor observation of other agents at all, 
(2) the team reward is defined as the mean of the agents’ individual rewards, and 
(3) only the team reward is used for training. 
There, agents need to learn from “reward-causing state-action pairs”, where the reward does not yield from the agents’ own actions but from the joint action of the team. The paper first shows that increasing the number of agents can increase the number of experiences of such reward-causing state-action pairs, allowing agents to learn more efficiently. However, the paper also shows that increasing the number of agents to infinity will cause the variance of the reward to converge to 0, leading to training failure. As a result, authors claim that there exist an optimal team size, which guarantees a minimal variance of the reward while allowing agents to experience reward-causing state-action pairs as much as possible. A series of experiments is conducted to support this conclusion. The paper is well-organized and easy to follow, and formulations/derivations are clear and correct under the assumptions made in the paper. However, the conclusion drawn in this paper (a too large team size may result in the failure of training) is somewhat a common sense for MARL. Although authors theoretically prove it by given some restrictive assumptions, the paper does not reveal how to find that optimal number of agents without exhaustive search, and thus the contribution of this paper appears rather limited and marginal.

(DTR) --> We consider the scenario without communication to study the influence of the team reward signal in isolation; however, we only use the mean team reward to be consistent with previous work. The team reward function can be any deterministic function and is not an assumption our work relies on in theory. We would also like to emphasize that we do not have the assumption that agents do not observe each other. We explore different amounts of observability, from no other-agent observations (4-states) to when all agents can be observed (Cleanup, NMMO) and find our theory scales to all of these scenarios. We do set the agents up as independent learners, so they do not share observations if that is what you are referencing (which is a common setup for independent RL, especially in mixed-motive environments).


3. Justification of the score
The contribution of this paper seems rather limited and marginal. This paper theoretically proves that there exists an optimal number of agents for MARL training under a certain environment assumption. However, it is rather common sense that too large a team will result in the failure of MARL training, while small teams make cooperation learning difficult. The real challenge surrounds how to find the near-optimal team size, without exhaustive search, and this is not discussed or addressed in the paper. Furthermore, the theoretical derivations made in this paper are based on rather restrictive assumptions (no communication/observations among agents, training only with team rewards), which are only met by few MARL problems.

(DTR) --> We would first like to highlight that the contribution you discuss here is only half of our paper's story. Section 4 provides theoretical motivations behind why teams could be leveraged to improve exploration and develop good policies (which has been recently shown empirically). This interplay where teammates can help agents explore has not been studied or properly understood previously. Focusing on your main point of credit assignment being common sense: we operate in the space of stochastic games (not Dec-POMDPs like VDN/QMIX that address credit assignment directly) to include more dynamics such as mixed-motive environments (such as the IPD and Cleanup environments). A common reward signal has been assumed to achieve the highest reward in mixed-motive environments; thus, it is often used to benchmark against (regardless of group size). Recent works have shown this is not necessarily true, but do not explore the underlying reasons. Our paper addresses open problems in this space from two directions: why teammates can be good in mixed-motive domains and why too many teammates can be bad (even in mixed-motive domains). We note that discovering these team structures is highly dependent on domain attributes but could be learned using a social planning agent (discussed in future work). The design of this social-planning agent needs to be properly motivated, which is one point of this paper. Lastly, we believe our assumptions are reasonable to explore the impacts of teams at the lowest level (i.e., communication adds further complexity of trust, possible deception, and incentives in mixed domains). We argue many real-world MARL problems share these characteristics, for example, there is currently no communication, shared observation, or coordinated pre-training in autonomous driving, especially across different manufacturers.


6. Questions for the author response.
In the experiment section, the mean of team rewards (TR) might not be a good metric to evaluate how good the trained policy is. As proved in the paper, TR will converge to 0 as the team size goes to infinity, so a relative larger team size is expected to result in a lower TR, regardless of the actual optimality of the policy. Instead, it would be more interesting to see a comparison between directly training and testing with a large team size and training with a smaller team size but testing with a larger team size, for example, in Cleanup task, training with 4 agents and testing with 7 agents, as opposed to a model that trained on 7 agents, so that the optimality of the policy can be compared fairly.

(DTR) --> It is important to note that Theorem 2 states the information of the reward signal will converge to 0, not the reward itself. This means a larger team is not necessarily expected to result in lower TR (i.e., Theorem 1 states more agents will increase the probability of getting non-zero reward in the first place). Your idea about training/testing with different team sizes is interesting within that context. However, the idea of this paper (and this line of work with multiagent teams) is to understand how teammates shape the environment for the development of policies, not how those agents work to coordinate in an ad hoc/testing scenario.


Reviewer #4 - Weak Accept (6)


3. Justification of the score
1) The main motivation of this paper is that smaller teams outperform larger teams (phenomenon). To motivate this phenomenon, the authors should take a concrete problem as an example, and show which learning algorithm will reveal such 
a counterintuitive phenomenon. All of these reinforcement learning algorithms will produce this phenomenon? 

(DTR) --> Our experiments deal with 3 different learning algorithms (Q-Learning, DQN, and PPO) with very different approaches (i.e., off-policy vs. on-policy, value-based vs. policy gradient). We show across 4 different environments that this phenomenon occurs. We will emphasize the generalization across learning algorithms in the camera ready and include a motivating example in the introduction.

2) The writing should be improved. There are many terminologies defined confusing. For example, in Section 3, 1st paragraph, the authors first assume agents have identical reward functions, i.e., $R_i=R_j$. However, in Eq.(1), the team reward is defined as the average rewards of teammates. It seems that the team rewards can be directly defined as $R_i$? Moreover, for different teams $T_i$ and $T_j$, how these agents behave at different teams respect to different reward functions. 

(DTR) --> Agents are defined to have identical reward functions before being placed in teams, meaning they receive the same rewards equally (e.g., they both get +1 for an apple in Cleanup). With teams, agents all share $TR_{i[n]}$ which replaces their individual reward function. We will clarify this notation in the camera ready.

3) In Section 4, the "reward-causing state action" should be defined clearly.

(DTR) --> We defined reward-causing state-action pairs using terminology from the RUDDER paper (where it is introduced); however, we will add a formalization to the camera ready version of the paper.

4) In Section 4, I am confused with the reward $R_{i}(s^t,a^t,s_{i}^{t})$. It states that all of the agents belongs to the same team can observe the whole environment in section 3. 

(DTR) --> Section 3 says that $S$ is able to be observed by all agents and agent $i$'s individually observed state is $s_i$, not fully observable. We introduce the term $R_{i}(s^t,a^t,s_{i}^{t})$ when explaining the reward dynamics of the 2-states environment conditioned on the individual next-state that $i$ transitions to (within the global state).

5) In experiments, in all of these three environments, there seems only one team, which is a special case of multiple teams studied in this paper. Why not just study the problem involving only one team in Sections 3 and 4.

(DTR) --> We empirically study single-team scenarios to remove any reward function impact from external teams in the testbed to properly measure the within-team impacts. However, our theory of within-team influences in Sections 3 and 4 generalizes to scenarios with multiple teams (such as the setting of multiple teams in past work).

4. Detailed feedback
In summary, this paper studies an interesting problem. However, the authors should validate the motivation of this counterintuitive phenomenon and improve the writing, such as define important symbols uniformly and concepts clearly.

(DTR) --> Our experiments in Cleanup and the IPD do validate the phenomenon found in previous work. We will include a motivating example in the introduction of the camera ready version.


Reviewer #5 - Weak Accept (6)

4. Detailed feedback

i) The reward sharing used in this paper is simple, i.e., Eq. (1). However, as the credit assignment is quite important for multi agent learning. The authors should add more justifications of the current choices of the reward sharing rule, as well as the discussion of other possible sharing rules, thus connecting to the widely used VDN or QMIX methods used in MARL.

(DTR) --> This is a good point. The reward sharing function is only required to be a deterministic function for our theory. We use mean team reward to be consistent with recent work in the context of teams and because do not limit our scope to Dec-POMDPs or the other assumptions listed around lines 92 - 95 (like VDN and QMIX). We consider stochastic game environment dynamics with fully independent learners where there may be mixed incentives and aligning agents' reward functions was previously thought to achieve the highest reward. We will emphasize these points to better show similarities/differences in the camera ready version.

ii) About the term "team structure", which is misleading. From my intuition, the team structure should be the relationship between agents, e.g., leader-follower relations, rather than the number and sizes of the teams. I would suggest to use a more concrete term, such team size and number. 

(DTR) --> We use ``team structure'' to be consistent with previous work within a similar context (probably inspired by ``network structure'' or "coalition structure"). We will consider changing this term in the camera ready for clarity.

iii) The implications of the theoretical results can be elaborated more. I would suggest the authors to add more discussion of the implications of the theoretical results, as well as the design of the cooperative MARL methods, which is of importance for researchers to appreciate the contributions of this paper.

(DTR) --> We will elaborate on these in the camera ready.

6. Questions for the author response.
Please discuss more about the rewarding sharing functions.

(DTR) --> The reward sharing function is only required to be a deterministic function for our theory. Our theory holds with any deterministic reward sharing function for a team. We use the mean team reward to be consistent with past work since we do not limit our environment to Dec-POMDPs with various pre-training and access assumptions (listed in lines 92 - 95). We are operating with individual learning agents in environments where there may be mixed incentives (and the dynamics of the environment are usually different in mixed settings like Cleanup or the IPD (appendix)).


==> Submit/IJCAI23-Submit/reviews.tex <==



Reviewer #1
Questions

1. Summary
The paper performs theoretical and empirical analysis on the effect of the team size in multi-agent learning the problems.
2. Score
Weak Accept (6)
3. Justification of the score
The paper is written well, performs an extensive theoretical and empirical analysis on three problems. Results support the conclusions.
4. Are the results in this paper easily reproducible ?
CONVINCING : I am convinced that the obtained results can be reproduced, possibly with some effort. Key resources (e.g., proofs, code, data) are already available, will be made available upon acceptance, or good reasons as to why they are not (e.g., proprietary data or code) are reported in the paper. Key details (e.g., proofs, experimental setup) are sufficiently well described but their exact recovery may require some work.
Reviewer #2
Questions

1. Summary
This paper studies an interesting and important problem in multiagent systems: how teams and different team structures influence and guide the learning process of individual agents. The authors theoretically show that the team improves the learning ability of respective agents by executing reward-causing state-action pairs more often and modifying the information variance. At the same time, the authors also prove that a large team faces a more challenging credit assignment problem than a small team as the information converges to 0 when team size increases. The empirical experiments also validate the proposed theory.
2. Score
Accept (7)
3. Justification of the score
1. This paper is well-organized and well-written.
2. The theoretical analysis is detailed and convincing. The conclusion drawn from the theory is interesting and important and may benefit the multiagent community.
3. The experiments are conducted in four environments and the results correspond to the proposed theory.
4. Detailed feedback
This paper derives an important conclusion that introducing teammates can help agents identify reward-causing state-action pairs, but too many teammates can make credit assignment more difficult which hinders learning. The analysis is step-by-step and supported by the theory, which is convincing.
5. Are the results in this paper easily reproducible ?
CONVINCING : I am convinced that the obtained results can be reproduced, possibly with some effort. Key resources (e.g., proofs, code, data) are already available, will be made available upon acceptance, or good reasons as to why they are not (e.g., proprietary data or code) are reported in the paper. Key details (e.g., proofs, experimental setup) are sufficiently well described but their exact recovery may require some work.
6. Questions for the author response.
There is a related work [1], which also studies in benefits of teams. As [1] works on the similar topic to this paper, it is encouraged to have more discussion with [1].

References
[1] Radke, D., Larson, K., & Brecht, T. Exploring the Benefits of Teams in Multiagent Learning. IJCAI, 2022.
Reviewer #3
Questions

1. Summary
This paper theoretically proves that there exists an optimal number of agents for MARL training under a certain environment assumption, where (1) there are no communication with nor observation of other agents at all, (2) the team reward is defined as the mean of the agents’ individual rewards, and (3) only the team reward is used for training. There, agents need to learn from “reward-causing state-action pairs”, where the reward does not yield from the agents’ own actions but from the joint action of the team. The paper first shows that increasing the number of agents can increase the number of experiences of such reward-causing state-action pairs, allowing agents to learn more efficiently. However, the paper also shows that increasing the number of agents to infinity will cause the variance of the reward to converge to 0, leading to training failure. As a result, authors claim that there exist an optimal team size, which guarantees a minimal variance of the reward while allowing agents to experience reward-causing state-action pairs as much as possible. A series of experiments is conducted to support this conclusion. The paper is well-organized and easy to follow, and formulations/derivations are clear and correct under the assumptions made in the paper. However, the conclusion drawn in this paper (a too large team size may result in the failure of training) is somewhat a common sense for MARL. Although authors theoretically prove it by given some restrictive assumptions, the paper does not reveal how to find that optimal number of agents without exhaustive search, and thus the contribution of this paper appears rather limited and marginal.
2. Score
Reject (4)
3. Justification of the score
The contribution of this paper seems rather limited and marginal. This paper theoretically proves that there exists an optimal number of agents for MARL training under a certain environment assumption. However, it is rather common sense that too large a team will result in the failure of MARL training, while small teams make cooperation learning difficult. The real challenge surrounds how to find the near-optimal team size, without exhaustive search, and this is not discussed or addressed in the paper. Furthermore, the theoretical derivations made in this paper are based on rather restrictive assumptions (no communication/observations among agents, training only with team rewards), which are only met by few MARL problems.
4. Detailed feedback
See my justification above.
5. Are the results in this paper easily reproducible ?
CONVINCING : I am convinced that the obtained results can be reproduced, possibly with some effort. Key resources (e.g., proofs, code, data) are already available, will be made available upon acceptance, or good reasons as to why they are not (e.g., proprietary data or code) are reported in the paper. Key details (e.g., proofs, experimental setup) are sufficiently well described but their exact recovery may require some work.
6. Questions for the author response.
In the experiment section, the mean of team rewards (TR) might not be a good metric to evaluate how good the trained policy is. As proved in the paper, TR will converge to 0 as the team size goes to infinity, so a relative larger team size is expected to result in a lower TR, regardless of the actual optimality of the policy. Instead, it would be more interesting to see a comparison between directly training and testing with a large team size and training with a smaller team size but testing with a larger team size, for example, in Cleanup task, training with 4 agents and testing with 7 agents, as opposed to a model that trained on 7 agents, so that the optimality of the policy can be compared fairly.
Reviewer #4
Questions

1. Summary
This paper aims to a better understanding of learning with multiagent systems, specially on why and which conditions, smaller teams outperform larger teams. To achieve this goal, this paper provides some theoretical analyzes, e.g., team structure and credit assignment on team performance. Experimental results are also conducted to validate their proposed analyzes.
2. Score
Weak Accept (6)
3. Justification of the score
1) The main motivation of this paper is that smaller teams outperform larger teams (phenomenon). To motivate this phenomenon, the authors should take a concrete problem as an example, and show which learning algorithm will reveal such 
a counterintuitive phenomenon. All of these reinforcement learning algorithms will produce this phenomenon? 
2) The writing should be improved. There are many terminologies defined confusing. For example, in Section 3, 1st paragraph, the authors first assume agents have identical reward functions, i.e., R_i=R_j. However, in Eq.(1), the team reward is defined as the average rewards of teammates. It seems that the team rewards can be directly defined as R_i? Moreover, for different teams T_i and T_j, how these agents behave at different teams respect to different reward functions. 
3) In Section 4, the "reward-causing state action" should be defined clearly.
4) In Section 4, I am confused with the reward R_{i}(s^t,a^t,s_{i}^{t}). It states that all of the agents belongs to the same team can observe the whole environment in section 3. 
5) In experiments, in all of these three environments, there seems only one team, which is a special case of multiple teams studied in this paper. Why not just study the problem involving only one team in Sections 3 and 4.
4. Detailed feedback
In summary, this paper studies an interesting problem. However, the authors should validate the motivation of this counterintuitive phenomenon and improve the writing, such as define important symbols uniformly and concepts clearly.
5. Are the results in this paper easily reproducible ?
CREDIBLE: I believe that the obtained results can, in principle, be reproduced. Even though key resources (e.g., proofs, code, data) are unavailable at this point, the key details (e.g., proof sketches, experimental setup) are sufficiently well described for an expert to confidently reproduce the main results, if given access to the missing resources.
6. Questions for the author response.
see Justification of the score
Reviewer #5
Questions

1. Summary
This paper considers the influence of the team structure on the cooperation learning for a population of individual learners.
2. Score
Weak Accept (6)
3. Justification of the score
This paper theoretically investigates how the teams structure can influence the learning of individual learners and the sub-optimal team structure will bring difficulties for the learning, and empirically validate the theoretical findings.
4. Detailed feedback
I generally think this is an interesting problem and the results are promising. Here are my main concerns: 

i) The reward sharing used in this paper is simple, i.e., Eq. (1). However, as the credit assignment is quite important for multi agent learning. The authors should add more justifications of the current choices of the reward sharing rule, as well as the discussion of other possible sharing rules, thus connecting to the widely used VDN or QMIX methods used in MARL. 

ii) About the term "team structure", which is misleading. From my intuition, the team structure should be the relationship between agents, e.g., leader-follower relations, rather than the number and sizes of the teams. I would suggest to use a more concrete term, such team size and number. 

iii) The implications of the theoretical results can be elaborated more. I would suggest the authors to add more discussion of the implications of the theoretical results, as well as the design of the cooperative MARL methods, which is of importance for researchers to appreciate the contributions of this paper.
5. Are the results in this paper easily reproducible ?
CREDIBLE: I believe that the obtained results can, in principle, be reproduced. Even though key resources (e.g., proofs, code, data) are unavailable at this point, the key details (e.g., proof sketches, experimental setup) are sufficiently well described for an expert to confidently reproduce the main results, if given access to the missing resources.
6. Questions for the author response.
Please discuss more about the rewarding sharing functions.

==> default_text.tex <==

\noindent Congratulations on having a paper selected for inclusion in an AAAI Press proceedings or technical report! This document details the requirements necessary to get your accepted paper published using PDF\LaTeX{}. If you are using Microsoft Word, instructions are provided in a different document. AAAI Press does not support any other formatting software.

The instructions herein are provided as a general guide for experienced \LaTeX{} users. If you do not know how to use \LaTeX{}, please obtain assistance locally. AAAI cannot provide you with support and the accompanying style files are \textbf{not} guaranteed to work. If the results you obtain are not in accordance with the specifications you received, you must correct your source file to achieve the correct result.

These instructions are generic. Consequently, they do not include specific dates, page charges, and so forth. Please consult your specific written conference instructions for details regarding your submission. Please review the entire document for specific instructions that might apply to your particular situation. All authors must comply with the following:

\begin{itemize}
\item You must use the 2022 AAAI Press \LaTeX{} style file and the aaai22.bst bibliography style files, which are located in the 2022 AAAI Author Kit (aaai22.sty, aaai22.bst).
\item You must complete, sign, and return by the deadline the AAAI copyright form (unless directed by AAAI Press to use the AAAI Distribution License instead).
\item You must read and format your paper source and PDF according to the formatting instructions for authors.
\item You must submit your electronic files and abstract using our electronic submission form \textbf{on time.}
\item You must pay any required page or formatting charges to AAAI Press so that they are received by the deadline.
\item You must check your paper before submitting it, ensuring that it compiles without error, and complies with the guidelines found in the AAAI Author Kit.
\end{itemize}

\section{Copyright}
All papers submitted for publication by AAAI Press must be accompanied by a valid signed copyright form. They must also contain the AAAI copyright notice at the bottom of the first page of the paper. There are no exceptions to these requirements. If you fail to provide us with a signed copyright form or disable the copyright notice, we will be unable to publish your paper. There are \textbf{no exceptions} to this policy. You will find a PDF version of the AAAI copyright form in the AAAI AuthorKit. Please see the specific instructions for your conference for submission details.

\section{Formatting Requirements in Brief}
We need source and PDF files that can be used in a variety of ways and can be output on a variety of devices. The design and appearance of the paper is strictly governed by the aaai style file (aaai22.sty).
\textbf{You must not make any changes to the aaai style file, nor use any commands, packages, style files, or macros within your own paper that alter that design, including, but not limited to spacing, floats, margins, fonts, font size, and appearance.} AAAI imposes requirements on your source and PDF files that must be followed. Most of these requirements are based on our efforts to standardize conference manuscript properties and layout. All papers submitted to AAAI for publication will be recompiled for standardization purposes. Consequently, every paper submission must comply with the following requirements:

\begin{itemize}
\item Your .tex file must compile in PDF\LaTeX{} --- (you may not include .ps or .eps figure files.)
\item All fonts must be embedded in the PDF file --- including your figures.
\item Modifications to the style file, whether directly or via commands in your document may not ever be made, most especially when made in an effort to avoid extra page charges or make your paper fit in a specific number of pages.
\item No type 3 fonts may be used (even in illustrations).
\item You may not alter the spacing above and below captions, figures, headings, and subheadings.
\item You may not alter the font sizes of text elements, footnotes, heading elements, captions, or title information (for references and mathematics, please see the limited exceptions provided herein).
\item You may not alter the line spacing of text.
\item Your title must follow Title Case capitalization rules (not sentence case).
\item Your .tex file must include completed metadata to pass-through to the PDF (see PDFINFO below).
\item \LaTeX{} documents must use the Times or Nimbus font package (you may not use Computer Modern for the text of your paper).
\item No \LaTeX{} 209 documents may be used or submitted.
\item Your source must not require use of fonts for non-Roman alphabets within the text itself. If your paper includes symbols in other languages (such as, but not limited to, Arabic, Chinese, Hebrew, Japanese, Thai, Russian and other Cyrillic languages), you must restrict their use to bit-mapped figures. Fonts that require non-English language support (CID and Identity-H) must be converted to outlines or 300 dpi bitmap or removed from the document (even if they are in a graphics file embedded in the document).
\item Two-column format in AAAI style is required for all papers.
\item The paper size for final submission must be US letter without exception.
\item The source file must exactly match the PDF.
\item The document margins may not be exceeded (no overfull boxes).
\item The number of pages and the file size must be as specified for your event.
\item No document may be password protected.
\item Neither the PDFs nor the source may contain any embedded links or bookmarks (no hyperref or navigator packages).
\item Your source and PDF must not have any page numbers, footers, or headers (no pagestyle commands).
\item Your PDF must be compatible with Acrobat 5 or higher.
\item Your \LaTeX{} source file (excluding references) must consist of a \textbf{single} file (use of the ``input" command is not allowed.
\item Your graphics must be sized appropriately outside of \LaTeX{} (do not use the ``clip" or ``trim'' command) .
\end{itemize}

If you do not follow these requirements, your paper will be returned to you to correct the deficiencies.

\section{What Files to Submit}
You must submit the following items to ensure that your paper is published:
\begin{itemize}
\item A fully-compliant PDF file that includes PDF metadata.
\item Your \LaTeX{} source file submitted as a \textbf{single} .tex file (do not use the ``input" command to include sections of your paper --- every section must be in the single source file). (The only allowable exception is .bib file, which should be included separately).
\item The bibliography (.bib) file(s).
\item Your source must compile on our system, which includes only standard \LaTeX{} 2020 TeXLive support files.
\item Only the graphics files used in compiling paper.
\item The \LaTeX{}-generated files (e.g. .aux,  .bbl file, PDF, etc.).
\end{itemize}

Your \LaTeX{} source will be reviewed and recompiled on our system (if it does not compile, your paper will be returned to you. \textbf{Do not submit your source in multiple text files.} Your single \LaTeX{} source file must include all your text, your bibliography (formatted using aaai22.bst), and any custom macros.

Your files should work without any supporting files (other than the program itself) on any computer with a standard \LaTeX{} distribution.

\textbf{Do not send files that are not actually used in the paper.} We don't want you to send us any files not needed for compiling your paper, including, for example, this instructions file, unused graphics files, style files, additional material sent for the purpose of the paper review, and so forth.

\textbf{Do not send supporting files that are not actually used in the paper.} We don't want you to send us any files not needed for compiling your paper, including, for example, this instructions file, unused graphics files, style files, additional material sent for the purpose of the paper review, and so forth.

\textbf{Obsolete style files.} The commands for some common packages (such as some used for algorithms), may have changed. Please be certain that you are not compiling your paper using old or obsolete style files.

\textbf{Final Archive.} Place your PDF and source files in a single archive which should be compressed using .zip. The final file size may not exceed 10 MB.
Name your source file with the last (family) name of the first author, even if that is not you.


\section{Using \LaTeX{} to Format Your Paper}

The latest version of the AAAI style file is available on AAAI's website. Download this file and place it in the \TeX\ search path. Placing it in the same directory as the paper should also work. You must download the latest version of the complete AAAI Author Kit so that you will have the latest instruction set and style file.

\subsection{Document Preamble}

In the \LaTeX{} source for your paper, you \textbf{must} place the following lines as shown in the example in this subsection. This command set-up is for three authors. Add or subtract author and address lines as necessary, and uncomment the portions that apply to you. In most instances, this is all you need to do to format your paper in the Times font. The helvet package will cause Helvetica to be used for sans serif. These files are part of the PSNFSS2e package, which is freely available from many Internet sites (and is often part of a standard installation).

Leave the setcounter for section number depth commented out and set at 0 unless you want to add section numbers to your paper. If you do add section numbers, you must uncomment this line and change the number to 1 (for section numbers), or 2 (for section and subsection numbers). The style file will not work properly with numbering of subsubsections, so do not use a number higher than 2.

\subsubsection{The Following Must Appear in Your Preamble}
\begin{quote}
\begin{scriptsize}\begin{verbatim}
\def\year{2022}\relax
\documentclass[letterpaper]{article}
% DO NOT CHANGE THIS
\usepackage{aaai22} % DO NOT CHANGE THIS
\usepackage{times} % DO NOT CHANGE THIS
\usepackage{helvet} % DO NOT CHANGE THIS
\usepackage{courier} % DO NOT CHANGE THIS
\usepackage[hyphens]{url} % DO NOT CHANGE THIS
\usepackage{graphicx} % DO NOT CHANGE THIS
\urlstyle{rm} % DO NOT CHANGE THIS
\def\UrlFont{\rm} % DO NOT CHANGE THIS
\usepackage{graphicx}  % DO NOT CHANGE THIS
\usepackage{natbib}  % DO NOT CHANGE THIS
\usepackage{caption}  % DO NOT CHANGE THIS
\DeclareCaptionStyle{ruled}%
  {labelfont=normalfont,labelsep=colon,strut=off}
\frenchspacing % DO NOT CHANGE THIS
\setlength{\pdfpagewidth}{8.5in} % DO NOT CHANGE THIS
\setlength{\pdfpageheight}{11in} % DO NOT CHANGE THIS
%
% PDF Info Is REQUIRED.
% For /Title, write your title in Mixed Case.
% Don't use accents or commands. Retain the parentheses.
% For /Author, add all authors within the parentheses,
% separated by commas. No accents, special characters
% or commands are allowed.
% Keep the /TemplateVersion tag as is
\pdfinfo{
/Title (AAAI Press Formatting Instructions for Authors
Using LaTeX -- A Guide)
/Author (AAAI Press Staff, Pater Patel Schneider,
Sunil Issar, J. Scott Penberthy, George Ferguson,
Hans Guesgen, Francisco Cruz, Marc Pujol-Gonzalez)
/TemplateVersion (2022.1)
}
\end{verbatim}\end{scriptsize}
\end{quote}

\subsection{Preparing Your Paper}

After the preamble above, you should prepare your paper as follows:
\begin{quote}
\begin{scriptsize}\begin{verbatim}
\begin{document}
\maketitle
\begin{abstract}
%...
\end{abstract}\end{verbatim}\end{scriptsize}
\end{quote}

\noindent You should then continue with the body of your paper. Your paper must conclude with the references, which should be inserted as follows:
\begin{quote}
\begin{scriptsize}\begin{verbatim}
% References and End of Paper
% These lines must be placed at the end of your paper
\bibliography{Bibliography-File}
\end{document}
\end{verbatim}\end{scriptsize}
\end{quote}

\subsection{Inserting Document Metadata with \LaTeX{}}
PDF files contain document summary information that enables us to create an Acrobat index (pdx) file, and also allows search engines to locate and present your paper more accurately. \textit{Document metadata for author and title are REQUIRED.} You may not apply any script or macro to the implementation of the title, author, and metadata information in your paper.

\textit{Important:} Do not include \textit{any} \LaTeX{} code or nonascii characters (including accented characters) in the metadata. The data in the metadata must be completely plain ascii. It may not include slashes, accents, linebreaks, unicode, or any \LaTeX{} commands. Type the title exactly as it appears on the paper (minus all formatting). Input the author names in the order in which they appear on the paper (minus all accents), separating each author by a comma. You may also include keywords in the optional Keywords field.

\begin{quote}
\begin{scriptsize}\begin{verbatim}
\begin{document}\\
\maketitle\\
...\\
\bibliography{Bibliography-File}\\
\end{document}\\
\end{verbatim}\end{scriptsize}
\end{quote}

\subsection{Commands and Packages That May Not Be Used}
\begin{table*}[t]
\centering

\begin{tabular}{l|l|l|l}
\textbackslash abovecaption &
\textbackslash abovedisplay &
\textbackslash addevensidemargin &
\textbackslash addsidemargin \\
\textbackslash addtolength &
\textbackslash baselinestretch &
\textbackslash belowcaption &
\textbackslash belowdisplay \\
\textbackslash break &
\textbackslash clearpage &
\textbackslash clip &
\textbackslash columnsep \\
\textbackslash float &
\textbackslash input &
\textbackslash input &
\textbackslash linespread \\
\textbackslash newpage &
\textbackslash pagebreak &
\textbackslash renewcommand &
\textbackslash setlength \\
\textbackslash text height &
\textbackslash tiny &
\textbackslash top margin &
\textbackslash trim \\
\textbackslash vskip\{- &
\textbackslash vspace\{- \\
\end{tabular}
%}
\caption{Commands that must not be used}
\label{table1}
\end{table*}

\begin{table}[t]
\centering
%\resizebox{.95\columnwidth}{!}{
\begin{tabular}{l|l|l|l}
    authblk & babel & cjk & dvips \\
    epsf & epsfig & euler & float \\
    fullpage & geometry & graphics & hyperref \\
    layout & linespread & lmodern & maltepaper \\
    navigator & pdfcomment & pgfplots & psfig \\
    pstricks & t1enc & titlesec & tocbind \\
    ulem
\end{tabular}
\caption{LaTeX style packages that must not be used.}
\label{table2}
\end{table}

There are a number of packages, commands, scripts, and macros that are incompatable with aaai22.sty. The common ones are listed in tables \ref{table1} and \ref{table2}. Generally, if a command, package, script, or macro alters floats, margins, fonts, sizing, linespacing, or the presentation of the references and citations, it is unacceptable. Note that negative vskip and vspace may not be used except in certain rare occurances, and may never be used around tables, figures, captions, sections, subsections, subsubsections, or references.


\subsection{Page Breaks}
For your final camera ready copy, you must not use any page break commands. References must flow directly after the text without breaks. Note that some conferences require references to be on a separate page during the review process. AAAI Press, however, does not require this condition for the final paper.


\subsection{Paper Size, Margins, and Column Width}
Papers must be formatted to print in two-column format on 8.5 x 11 inch US letter-sized paper. The margins must be exactly as follows:
\begin{itemize}
\item Top margin: .75 inches
\item Left margin: .75 inches
\item Right margin: .75 inches
\item Bottom margin: 1.25 inches
\end{itemize}


The default paper size in most installations of \LaTeX{} is A4. However, because we require that your electronic paper be formatted in US letter size, the preamble we have provided includes commands that alter the default to US letter size. Please note that using any other package to alter page size (such as, but not limited to the Geometry package) will result in your final paper being returned to you for correction.


\subsubsection{Column Width and Margins.}
To ensure maximum readability, your paper must include two columns. Each column should be 3.3 inches wide (slightly more than 3.25 inches), with a .375 inch (.952 cm) gutter of white space between the two columns. The aaai22.sty file will automatically create these columns for you.

\subsection{Overlength Papers}
If your paper is too long and you resort to formatting tricks to make it fit, it is quite likely that it will be returned to you. The best way to retain readability if the paper is overlength is to cut text, figures, or tables. There are a few acceptable ways to reduce paper size that don't affect readability. First, turn on \textbackslash frenchspacing, which will reduce the space after periods. Next, move all your figures and tables to the top of the page. Consider removing less important portions of a figure. If you use \textbackslash centering instead of \textbackslash begin\{center\} in your figure environment, you can also buy some space. For mathematical environments, you may reduce fontsize {\bf but not below 6.5 point}.


Commands that alter page layout are forbidden. These include \textbackslash columnsep,  \textbackslash float, \textbackslash topmargin, \textbackslash topskip, \textbackslash textheight, \textbackslash textwidth, \textbackslash oddsidemargin, and \textbackslash evensizemargin (this list is not exhaustive). If you alter page layout, you will be required to pay the page fee. Other commands that are questionable and may cause your paper to be rejected include \textbackslash parindent, and \textbackslash parskip. Commands that alter the space between sections are forbidden. The title sec package is not allowed. Regardless of the above, if your paper is obviously ``squeezed" it is not going to to be accepted. Options for reducing the length of a paper include reducing the size of your graphics, cutting text, or paying the extra page charge (if it is offered).


\subsection{Type Font and Size}
Your paper must be formatted in Times Roman or Nimbus. We will not accept papers formatted using Computer Modern or Palatino or some other font as the text or heading typeface. Sans serif, when used, should be Courier. Use Symbol or Lucida or Computer Modern for \textit{mathematics only. }

Do not use type 3 fonts for any portion of your paper, including graphics. Type 3 bitmapped fonts are designed for fixed resolution printers. Most print at 300 dpi even if the printer resolution is 1200 dpi or higher. They also often cause high resolution imagesetter devices to crash. Consequently, AAAI will not accept electronic files containing obsolete type 3 fonts. Files containing those fonts (even in graphics) will be rejected. (Authors using blackboard symbols must be avoid those packages that use type 3 fonts.)

Fortunately, there are effective workarounds that will prevent your file from embedding type 3 bitmapped fonts. The easiest workaround is to use the required times, helvet, and courier packages with \LaTeX{}2e. (Note that papers formatted in this way will still use Computer Modern for the mathematics. To make the math look good, you'll either have to use Symbol or Lucida, or you will need to install type 1 Computer Modern fonts --- for more on these fonts, see the section ``Obtaining Type 1 Computer Modern.")

If you are unsure if your paper contains type 3 fonts, view the PDF in Acrobat Reader. The Properties/Fonts window will display the font name, font type, and encoding properties of all the fonts in the document. If you are unsure if your graphics contain type 3 fonts (and they are PostScript or encapsulated PostScript documents), create PDF versions of them, and consult the properties window in Acrobat Reader.

The default size for your type must be ten-point with twelve-point leading (line spacing). Start all pages (except the first) directly under the top margin. (See the next section for instructions on formatting the title page.) Indent ten points when beginning a new paragraph, unless the paragraph begins directly below a heading or subheading.


\subsubsection{Obtaining Type 1 Computer Modern for \LaTeX{}.}

If you use Computer Modern for the mathematics in your paper (you cannot use it for the text) you may need to download type 1 Computer fonts. They are available without charge from the American Mathematical Society:
http://www.ams.org/tex/type1-fonts.html.

\subsubsection{Nonroman Fonts.}
If your paper includes symbols in other languages (such as, but not limited to, Arabic, Chinese, Hebrew, Japanese, Thai, Russian and other Cyrillic languages), you must restrict their use to bit-mapped figures.

\subsection{Title and Authors}
Your title must appear in mixed case (nouns, pronouns, and verbs are capitalized) near the top of the first page, centered over both columns in sixteen-point bold type (twenty-four point leading). This style is called ``mixed case" (or ``title case"), which means that all verbs (including short verbs like be, is, using, and go), nouns, adverbs, adjectives, and pronouns should be capitalized, (including both words in hyphenated terms), while articles, conjunctions, and prepositions are lower case unless they directly follow a colon or long dash.

Author's names should appear below the title of the paper, centered in twelve-point type (with fifteen point leading), along with affiliation(s) and complete address(es) (including electronic mail address if available) in nine-point roman type (the twelve point leading). You should begin the two-column format when you come to the abstract.

\subsubsection{Formatting Author Information.}
Author information has to be set according the following specification depending if you have one or more than one affiliation.  You may not use a table nor may you employ the \textbackslash authorblk.sty package. For one or several authors from the same institution, please just separate with commas and write the affiliation directly below using the macros \textbackslash author and \textbackslash affiliations:

\begin{quote}\begin{scriptsize}\begin{verbatim}
\author{
    Author 1, ..., Author n\\
}
\affiliations {
    Address line\\
    ... \\
    Address line\\
}
\end{verbatim}\end{scriptsize}\end{quote}


\noindent For authors from different institutions, use \textbackslash textsuperscript \{\textbackslash rm x \} to match authors and affiliations. Notice that there should not be any spaces between the author name (or comma following it) and the superscript.

\begin{quote}\begin{scriptsize}\begin{verbatim}
\author{
    AuthorOne,\equalcontrib\textsuperscript{\rm 1}
    AuthorTwo,\equalcontrib\textsuperscript{\rm 2}
    AuthorThree,\textsuperscript{\rm 3}\\
    AuthorFour,\textsuperscript{\rm 4}
    AuthorFive \textsuperscript{\rm 5}}
}
\affiliations {
    \textsuperscript{\rm 1}AffiliationOne,\\
    \textsuperscript{\rm 2}AffiliationTwo,\\
    \textsuperscript{\rm 3}AffiliationThree,\\
    \textsuperscript{\rm 4}AffiliationFour,\\
    \textsuperscript{\rm 5}AffiliationFive\\
    \{email, email\}@affiliation.com,
    email@affiliation.com,
    email@affiliation.com,
    email@affiliation.com
}
\end{verbatim}\end{scriptsize}\end{quote}

You can indicate that some authors contributed equally using the \textbackslash equalcontrib command. This will add a marker after the author names and a footnote on the first page.

Note that you may want to  break the author list for better visualization. You can achieve this using a simple line break (\textbackslash  \textbackslash).

\subsection{\LaTeX{} Copyright Notice}
The copyright notice automatically appears if you use aaai22.sty. It has been hardcoded and may not be disabled.

\subsection{Credits}
Any credits to a sponsoring agency should appear in the acknowledgments section, unless the agency requires different placement. If it is necessary to include this information on the front page, use
\textbackslash thanks in either the \textbackslash author or \textbackslash title commands.
For example:
\begin{quote}
\begin{small}
\textbackslash title\{Very Important Results in AI\textbackslash thanks\{This work is
 supported by everybody.\}\}
\end{small}
\end{quote}
Multiple \textbackslash thanks commands can be given. Each will result in a separate footnote indication in the author or title with the corresponding text at the botton of the first column of the document. Note that the \textbackslash thanks command is fragile. You will need to use \textbackslash protect.

Please do not include \textbackslash pubnote commands in your document.

\subsection{Abstract}
Follow the example commands in this document for creation of your abstract. The command \textbackslash begin\{abstract\} will automatically indent the text block. Please do not indent it further. {Do not include references in your abstract!}

\subsection{Page Numbers}

Do not \textbf{ever} print any page numbers on your paper. The use of \textbackslash pagestyle is forbidden.

\subsection{Text }
The main body of the paper must be formatted in black, ten-point Times Roman with twelve-point leading (line spacing). You may not reduce font size or the linespacing. Commands that alter font size or line spacing (including, but not limited to baselinestretch, baselineshift, linespread, and others) are expressly forbidden. In addition, you may not use color in the text.

\subsection{Citations}
Citations within the text should include the author's last name and year, for example (Newell 1980). Append lower-case letters to the year in cases of ambiguity. Multiple authors should be treated as follows: (Feigenbaum and Engelmore 1988) or (Ford, Hayes, and Glymour 1992). In the case of four or more authors, list only the first author, followed by et al. (Ford et al. 1997).

\subsection{Extracts}
Long quotations and extracts should be indented ten points from the left and right margins.

\begin{quote}
This is an example of an extract or quotation. Note the indent on both sides. Quotation marks are not necessary if you offset the text in a block like this, and properly identify and cite the quotation in the text.

\end{quote}

\subsection{Footnotes}
Avoid footnotes as much as possible; they interrupt the reading of the text. When essential, they should be consecutively numbered throughout with superscript Arabic numbers. Footnotes should appear at the bottom of the page, separated from the text by a blank line space and a thin, half-point rule.

\subsection{Headings and Sections}
When necessary, headings should be used to separate major sections of your paper. Remember, you are writing a short paper, not a lengthy book! An overabundance of headings will tend to make your paper look more like an outline than a paper. The aaai22.sty package will create headings for you. Do not alter their size nor their spacing above or below.

\subsubsection{Section Numbers.}
The use of section numbers in AAAI Press papers is optional. To use section numbers in \LaTeX{}, uncomment the setcounter line in your document preamble and change the 0 to a 1. Section numbers should not be used in short poster papers and/or extended abstracts.

\subsubsection{Section Headings.}
Sections should be arranged and headed as follows:
\begin{enumerate}
\item Main content sections
\item Appendices (optional)
\item Ethical statement (optional, unnumbered)
\item Acknowledgements (optional, unnumbered)
\item References (unnumbered)
\end{enumerate}

\subsubsection{Appendices.}
Any appendices must appear after the main content. If your main sections are numbered, appendix sections must use letters instead of arabic numerals. In \LaTeX{} you can use the \texttt{\textbackslash appendix} command to achieve this effect and then use \texttt{\textbackslash section\{Heading\}} normally for your appendix sections.

\subsubsection{Ethical statement.}
You can write a statement about the potential ethical impact of your work, including its broad societal implications, both positive and negative. If included, such statement must be written in an unnumbered section titled \emph{Ethical statement}.

\subsubsection{Acknowledgments.}
The acknowledgments section, if included, appears right before the references and is headed ``Acknowledgments". It must not be numbered even if other sections are (use \texttt{\textbackslash section*\{Acknowledgements\}} in \LaTeX{}). This section includes acknowledgments of help from associates and colleagues, credits to sponsoring agencies, financial support, and permission to publish. Please acknowledge other contributors, grant support, and so forth, in this section. Do not put acknowledgments in a footnote on the first page. If your grant agency requires acknowledgment of the grant on page 1, limit the footnote to the required statement, and put the remaining acknowledgments at the back. Please try to limit acknowledgments to no more than three sentences.

\subsubsection{References.}
The references section should be labeled ``References" and must appear at the very end of the paper (don't end the paper with references, and then put a figure by itself on the last page). A sample list of references is given later on in these instructions. Please use a consistent format for references. Poorly prepared or sloppy references reflect badly on the quality of your paper and your research. Please prepare complete and accurate citations.

\subsection{Illustrations and  Figures}

\begin{figure}[t]
\centering
\includegraphics[width=0.9\columnwidth]{figure1} % Reduce the figure size so that it is slightly narrower than the column. Don't use precise values for figure width.This setup will avoid overfull boxes.
\caption{Using the trim and clip commands produces fragile layers that can result in disasters (like this one from an actual paper) when the color space is corrected or the PDF combined with others for the final proceedings. Crop your figures properly in a graphics program -- not in LaTeX}.
\label{fig1}
\end{figure}

\begin{figure*}[t]
\centering
\includegraphics[width=0.8\textwidth]{figure2} % Reduce the figure size so that it is slightly narrower than the column.
\caption{Adjusting the bounding box instead of actually removing the unwanted data resulted multiple layers in this paper. It also needlessly increased the PDF size. In this case, the size of the unwanted layer doubled the paper's size, and produced the following surprising results in final production. Crop your figures properly in a graphics program. Don't just alter the bounding box.}
\label{fig2}
\end{figure*}

% Using the \centering command instead of \begin{center} ... \end{center} will save space
% Positioning your figure at the top of the page will save space and make the paper more readable
% Using 0.95\columnwidth in conjunction with the


Your paper must compile in PDF\LaTeX{}. Consequently, all your figures must be .jpg, .png, or .pdf. You may not use the .gif (the resolution is too low), .ps, or .eps file format for your figures.

Figures, drawings, tables, and photographs should be placed throughout the paper on the page (or the subsequent page) where they are first discussed. Do not group them together at the end of the paper. If placed at the top of the paper, illustrations may run across both columns. Figures must not invade the top, bottom, or side margin areas. Figures must be inserted using the \textbackslash usepackage\{graphicx\}. Number figures sequentially, for example, figure 1, and so on. Do not use minipage to group figures.

If you normally create your figures using pgfplots, please create the figures first, and then import them as pdfs with proper bounding boxes, as the bounding and trim boxes created by pfgplots are fragile and not valid.

When you include your figures, you must crop them \textbf{outside} of \LaTeX{}. The command \textbackslash includegraphics*[clip=true, viewport 0 0 10 10]{...} might result in a PDF that looks great, but the image is \textbf{not really cropped.} The full image can reappear (and obscure whatever it is overlapping) when page numbers are applied or color space is standardized. Figures \ref{fig1}, and \ref{fig2} display some unwanted results that often occur.

If your paper includes illustrations that are not compatible with PDF\TeX{} (such as .eps or .ps documents), you will need to convert them. The epstopdf package will usually work for eps files. You will need to convert your ps files to PDF in either case.

\subsubsection {Figure Captions.}The illustration number and caption must appear \textit{under} the illustration. Labels and other text with the actual illustration must be at least nine-point type. However, the font and size of figure captions must be 10 point roman. Do not make them smaller, bold, or italic. (Individual words may be italicized if the context requires differentiation.)

\subsection{Tables}

Tables should be presented in 10 point roman type. If necessary, they may be altered to 9 point type. You may not use any commands that further reduce point size below nine points. Tables that do not fit in a single column must be placed across double columns. If your table won't fit within the margins even when spanning both columns, you must split it. Do not use minipage to group tables.

\subsubsection {Table Captions.} The number and caption for your table must appear \textit{under} (not above) the table.  Additionally, the font and size of table captions must be 10 point roman and must be placed beneath the figure. Do not make them smaller, bold, or italic. (Individual words may be italicized if the context requires differentiation.)



\subsubsection{Low-Resolution Bitmaps.}
You may not use low-resolution (such as 72 dpi) screen-dumps and GIF files---these files contain so few pixels that they are always blurry, and illegible when printed. If they are color, they will become an indecipherable mess when converted to black and white. This is always the case with gif files, which should never be used. The resolution of screen dumps can be increased by reducing the print size of the original file while retaining the same number of pixels. You can also enlarge files by manipulating them in software such as PhotoShop. Your figures should be 300 dpi when incorporated into your document.

\subsubsection{\LaTeX{} Overflow.}
\LaTeX{} users please beware: \LaTeX{} will sometimes put portions of the figure or table or an equation in the margin. If this happens, you need to make the figure or table span both columns. If absolutely necessary, you may reduce the figure, or reformat the equation, or reconfigure the table.{ \bf Check your log file!} You must fix any overflow into the margin (that means no overfull boxes in \LaTeX{}). \textbf{Nothing is permitted to intrude into the margin or gutter.}


\subsubsection{Using Color.}
Use of color is restricted to figures only. It must be WACG 2.0 compliant. (That is, the contrast ratio must be greater than 4.5:1 no matter the font size.) It must be CMYK, NOT RGB. It may never be used for any portion of the text of your paper. The archival version of your paper will be printed in black and white and grayscale. The web version must be readable by persons with disabilities. Consequently, because conversion to grayscale can cause undesirable effects (red changes to black, yellow can disappear, and so forth), we strongly suggest you avoid placing color figures in your document. If you do include color figures, you must (1) use the CMYK (not RGB) colorspace and (2) be mindful of readers who may happen to have trouble distinguishing colors. Your paper must be decipherable without using color for distinction.

\subsubsection{Drawings.}
We suggest you use computer drawing software (such as Adobe Illustrator or, (if unavoidable), the drawing tools in Microsoft Word) to create your illustrations. Do not use Microsoft Publisher. These illustrations will look best if all line widths are uniform (half- to two-point in size), and you do not create labels over shaded areas. Shading should be 133 lines per inch if possible. Use Times Roman or Helvetica for all figure call-outs. \textbf{Do not use hairline width lines} --- be sure that the stroke width of all lines is at least .5 pt. Zero point lines will print on a laser printer, but will completely disappear on the high-resolution devices used by our printers.

\subsubsection{Photographs and Images.}
Photographs and other images should be in grayscale (color photographs will not reproduce well; for example, red tones will reproduce as black, yellow may turn to white, and so forth) and set to a minimum of 300 dpi. Do not prescreen images.

\subsubsection{Resizing Graphics.}
Resize your graphics \textbf{before} you include them with LaTeX. You may \textbf{not} use trim or clip options as part of your \textbackslash includegraphics command. Resize the media box of your PDF using a graphics program instead.

\subsubsection{Fonts in Your Illustrations.}
You must embed all fonts in your graphics before including them in your LaTeX document.

\subsubsection{Algorithms.}
Algorithms and/or programs are a special kind of figures. Like all illustrations, they should appear floated to the top (preferably) or bottom of the page. However, their caption should appear in the header, left-justified and enclosed between horizontal lines, as shown in Algorithm~\ref{alg:algorithm}. The algorithm body should be terminated with another horizontal line. It is up to the authors to decide whether to show line numbers or not, how to format comments, etc.

In \LaTeX{} algorithms may be typeset using the {\tt algorithm} and {\tt algorithmic} packages, but you can also use one of the many other packages for the task.

\begin{algorithm}[tb]
\caption{Example algorithm}
\label{alg:algorithm}
\textbf{Input}: Your algorithm's input\\
\textbf{Parameter}: Optional list of parameters\\
\textbf{Output}: Your algorithm's output
\begin{algorithmic}[1] %[1] enables line numbers
\STATE Let $t=0$.
\WHILE{condition}
\STATE Do some action.
\IF {conditional}
\STATE Perform task A.
\ELSE
\STATE Perform task B.
\ENDIF
\ENDWHILE
\STATE \textbf{return} solution
\end{algorithmic}
\end{algorithm}

\subsubsection{Listings.}
Listings are much like algorithms and programs. They should also appear floated to the top (preferably) or bottom of the page. Listing captions should appear in the header, left-justified and enclosed between horizontal lines as shown in Listing~\ref{lst:listing}. Terminate the body with another horizontal line and avoid any background color. Line numbers, if included, must appear within the text column.

\begin{listing}[tb]%
\caption{Example listing {\tt quicksort.hs}}%
\label{lst:listing}%
\begin{lstlisting}[language=Haskell]
quicksort :: Ord a => [a] -> [a]
quicksort []     = []
quicksort (p:xs) = (quicksort lesser) ++ [p] ++ (quicksort greater)
	where
		lesser  = filter (< p) xs
		greater = filter (>= p) xs
\end{lstlisting}
\end{listing}

\subsection{References}
The AAAI style includes a set of definitions for use in formatting references with BibTeX. These definitions make the bibliography style fairly close to the ones  specified in the Reference Examples appendix below. To use these definitions, you also need the BibTeX style file ``aaai22.bst," available in the AAAI Author Kit on the AAAI web site. Then, at the end of your paper but before \textbackslash end{document}, you need to put the following lines:

\begin{quote}
\begin{small}
\textbackslash bibliography\{bibfile1,bibfile2,...\}
\end{small}
\end{quote}

Please note that the aaai22.sty class already sets the bibliographystyle for you, so you do not have to place any \textbackslash bibliographystyle command in the document yourselves. The aaai22.sty file is incompatible with the hyperref and navigator packages. If you use either, your references will be garbled and your paper will be returned to you.

References may be the same size as surrounding text. However, in this section (only), you may reduce the size to \textbackslash small if your paper exceeds the allowable number of pages. Making it any smaller than 9 point with 10 point linespacing, however, is not allowed. A more precise and exact method of reducing the size of your references minimally is by means of the following command: \begin{quote}
\textbackslash fontsize\{9.8pt\}\{10.8pt\}
\textbackslash selectfont\end{quote}

\noindent You must reduce the size equally for both font size and line spacing, and may not reduce the size beyond \{9.0pt\}\{10.0pt\}.

The list of files in the \textbackslash bibliography command should be the names of your BibTeX source files (that is, the .bib files referenced in your paper).

The following commands are available for your use in citing references:
\begin{quote}
{\em \textbackslash cite:} Cites the given reference(s) with a full citation. This appears as ``(Author Year)'' for one reference, or ``(Author Year; Author Year)'' for multiple references.\smallskip\\
{\em \textbackslash shortcite:} Cites the given reference(s) with just the year. This appears as ``(Year)'' for one reference, or ``(Year; Year)'' for multiple references.\smallskip\\
{\em \textbackslash citeauthor:} Cites the given reference(s) with just the author name(s) and no parentheses.\smallskip\\
{\em \textbackslash citeyear:} Cites the given reference(s) with just the date(s) and no parentheses.
\end{quote}
You may also use any of the \emph{natbib} citation commands.


\section{Proofreading Your PDF}
Please check all the pages of your PDF file. The most commonly forgotten element is the acknowledgements --- especially the correct grant number. Authors also commonly forget to add the metadata to the source, use the wrong reference style file, or don't follow the capitalization rules or comma placement for their author-title information properly. A final common problem is text (expecially equations) that runs into the margin. You will need to fix these common errors before submitting your file.

\section{Improperly Formatted Files }
In the past, AAAI has corrected improperly formatted files submitted by the authors. Unfortunately, this has become an increasingly burdensome expense that we can no longer absorb). Consequently, if your file is improperly formatted, it will be returned to you for correction.

\subsection{\LaTeX{} 209 Warning}
If you use \LaTeX{} 209 your paper will be returned to you unpublished. Convert your paper to \LaTeX{}2e.

\section{Naming Your Electronic File}
We require that you name your \LaTeX{} source file with the last name (family name) of the first author so that it can easily be differentiated from other submissions. Complete file-naming instructions will be provided to you in the submission instructions.

\section{Submitting Your Electronic Files to AAAI}
Instructions on paper submittal will be provided to you in your acceptance letter.

\section{Inquiries}
If you have any questions about the preparation or submission of your paper as instructed in this document, please contact AAAI Press at the address given below. If you have technical questions about implementation of the aaai style file, please contact an expert at your site. We do not provide technical support for \LaTeX{} or any other software package. To avoid problems, please keep your paper simple, and do not incorporate complicated macros and style files.

\begin{quote}
\noindent AAAI Press\\
2275 East Bayshore Road, Suite 160\\
Palo Alto, California 94303\\
\textit{Telephone:} (650) 328-3123\\
\textit{E-mail:} See the submission instructions for your particular conference or event.
\end{quote}

\section{Additional Resources}
\LaTeX{} is a difficult program to master. If you've used that software, and this document didn't help or some items were not explained clearly, we recommend you read Michael Shell's excellent document (testflow doc.txt V1.0a 2002/08/13) about obtaining correct PS/PDF output on \LaTeX{} systems. (It was written for another purpose, but it has general application as well). It is available at www.ctan.org in the tex-archive.

\appendix
\section{Reference Examples}
\label{sec:reference_examples}

\nobibliography*
Formatted bibliographies should look like the following examples. You should use BibTeX to generate the references. Missing fields are unacceptable when compiling references, and usually indicate that you are using the wrong type of entry (BibTeX class).

\paragraph{Book with multiple authors~\nocite{em:86}} Use the \texttt{@book} class.\\[.2em]
\bibentry{em:86}.

\paragraph{Journal and magazine articles~\nocite{r:80, hcr:83}} Use the \texttt{@article} class.\\[.2em]
\bibentry{r:80}.\\[.2em]
\bibentry{hcr:83}.

\paragraph{Proceedings paper published by a society, press or publisher~\nocite{c:83, c:84}} Use the \texttt{@inproceedings} class. You may abbreviate the \emph{booktitle} field, but make sure that the conference edition is clear.\\[.2em]
\bibentry{c:84}.\\[.2em]
\bibentry{c:83}.

\paragraph{University technical report~\nocite{r:86}} Use the \texttt{@techreport} class.\\[.2em]
\bibentry{r:86}.

\paragraph{Dissertation or thesis~\nocite{c:79}} Use the \texttt{@phdthesis} class.\\[.2em]
\bibentry{c:79}.

\paragraph{Forthcoming publication~\nocite{c:21}} Use the \texttt{@misc} class with a \texttt{note="Forthcoming"} annotation.
\begin{quote}
\begin{footnotesize}
\begin{verbatim}
@misc(key,
  [...]
  note="Forthcoming",
)
\end{verbatim}
\end{footnotesize}
\end{quote}
\bibentry{c:21}.

\paragraph{ArXiv paper~\nocite{c:22}} Fetch the BibTeX entry from the "Export Bibtex Citation" link in the arXiv website. Notice it uses the \texttt{@misc} class instead of the \texttt{@article} one, and that it includes the \texttt{eprint} and \texttt{archivePrefix} keys.
\begin{quote}
\begin{footnotesize}
\begin{verbatim}
@misc(key,
  [...]
  eprint="xxxx.yyyy",
  archivePrefix="arXiv",
)
\end{verbatim}
\end{footnotesize}
\end{quote}
\bibentry{c:22}.

\paragraph{Website or online resource~\nocite{c:23}} Use the \texttt{@misc} class. Add the url in the \texttt{howpublished} field and the date of access in the \texttt{note} field:
\begin{quote}
\begin{footnotesize}
\begin{verbatim}
@misc(key,
  [...]
  howpublished="\url{http://...}",
  note="Accessed: YYYY-mm-dd",
)
\end{verbatim}
\end{footnotesize}
\end{quote}
\bibentry{c:23}.

\vspace{.2em}
For the most up to date version of the AAAI reference style, please consult the \textit{AI Magazine} Author Guidelines at \url{https://aaai.org/ojs/index.php/aimagazine/about/submissions#authorGuidelines}

% Use \bibliography{yourbibfile} instead or the References section will not appear in your paper
\nobibliography{aaai22}

\section{Acknowledgments}
AAAI is especially grateful to Peter Patel Schneider for his work in implementing the original aaai.sty file, liberally using the ideas of other style hackers, including Barbara Beeton. We also acknowledge with thanks the work of George Ferguson for his guide to using the style and BibTeX files --- which has been incorporated into this document --- and Hans Guesgen, who provided several timely modifications, as well as the many others who have, from time to time, sent in suggestions on improvements to the AAAI style. We are especially grateful to Francisco Cruz, Marc Pujol-Gonzalez, and Mico Loretan for the improvements to the Bib\TeX{} and \LaTeX{} files made in 2020.

The preparation of the \LaTeX{} and Bib\TeX{} files that implement these instructions was supported by Schlumberger Palo Alto Research, AT\&T Bell Laboratories, Morgan Kaufmann Publishers, The Live Oak Press, LLC, and AAAI Press. Bibliography style changes were added by Sunil Issar. \verb+\+pubnote was added by J. Scott Penberthy. George Ferguson added support for printing the AAAI copyright slug. Additional changes to aaai22.sty and aaai22.bst have been made by Francisco Cruz, Marc Pujol-Gonzalez, and Mico Loretan.

\bigskip
\noindent Thank you for reading these instructions carefully. We look forward to receiving your electronic files!


==> increase_reward_distribution.tex <==
% \subsection{Positives of Increasing Team Size}
% \section{Benefits of Teams}
% \label{sec:pos_team_size}

\section{Teams as Autonomous Reward Redistributors}
\label{sec:increase_reward_dist}

% As teams increase in size, the variance of the reward distribution across states increases.
% This improves the ability for agents to identify conditional states where ``jumps'' in the value function must be learned (like in RUDDER).
% Some thoughts:

% \begin{itemize}
%     \item Similar to goals in hierarchical learning and options in single-agent environments. Learning one sub-goal should be easier than learning whole trajectory (options).
    
%     \item Agents achieving these goals creates an autocurricula for their teammates (spreading reward among the team at different states means agents learn about their own sub-goals better. The culmination leads to more efficiency of the entire environment).
    
%     \item Effectiveness is determined by environment. If there is one conditional state, fewer agents needed than if there are 4 conditional states.
% \end{itemize}


% \\\\\\\

% Rudder: redistribution transforms RL task to regression task (deciding which state/action pairs should get which reward). Teams complete this regression task already, doesn't need to be learned by single agent. Learning regression in rudder requires completed trajectories... teams do not.

% "changing the reward changes the optimal policies" (rudder paper)... learning roles are not optimal in the single agent sense, but optimal in multiagent sense... different problem

% Do teams create an SDP for for stochastic games? Expected reward should be equivalent, but not sure this is best way to talk about this.

% \newtext{Actual text below:}

% \todo{I talk about states, but these might need to be state-action pairs. Thoughts? These paragraphs may also be redundant from related work.}

% In sparse or delayed-reward RL tasks, states that are important for high overall return may not actually offer immediate environmental reward.


In this section, we are interested in the redistribution of exogenous rewards to particular reward-causing state-action pairs that are individually observed by individual agents.
Therefore, we analyze the team-based reward agent $i$ receives when they transition to an individually observed state $s_i$ (which contributes to the joint state $s^t$).

In single agent RL, an agent needs to learn that state $s_c$ is valuable despite the lack of exogenous reward -- a difficult problem in certain conditions.
Using reward redistribution algorithms, agents shift the distribution of their sequence-associated return across their experiences to help learn about relevant reward-causing state-action pairs in their memory~\cite{arjona2019rudder}.
With multiagent teams where $n > 1$, reward redistribution happens between agents instantaneously through the shared team-based reward channel.
Thus, reward-causing state-action pairs can be perceived to actually provide reward if $i$'s teammates obtain the exogenous reward these state-action pairs cause elsewhere.

We investigate the relationship between team structure and reward redistribution across individually observed state-action pairs using our example SG shown in Figure~\ref{fig:2_states}.
Critical to our analysis, we study the \emph{expected} team-based reward that agents in $T_i$ receive for executing reward-causing state-action pairs.
As stated previously, we assume agents are initialized randomly at the beginning of learning and cover the state space.
This lends itself to calculating the expectation as the mean value over all possible state-action pairs assuming equal likelihood.
% The expectation assumes agents perform random walks and cover the state space uniformly at random, analogous to newly instantiated agents at the beginning of training which is consistent with past work~\cite{arumugam2021information}.
Reward redistribution then shapes the environment which ultimately impacts the following learning process.

In our example, visiting $s_c$ is a general example of a reward-causing state-action pair since the binary signal $c$ that determines the reward at $s_r$ is dependent on visiting $s_c$.
We first show how the expected team-based reward that agents receive when they individually visit $s_c$ increases as a function of team size (i.e., increasing team size leads to more perceived reward when visiting $s_c$).




% We investigate the relationship between team structure and reward redistribution in our example SG environment.
% We provide insight as to how increasing the size of a team $n$ redistributes reward to alternative reward-causing state-action pairs which may not yield exogenous reward.
% This process can be thought of as being similar to forming sub-goals in single-agent RL; however, sub-goals are created by agents for their teammates to achieve.
% As a result, the expected reward for valuable state-action pairs increases and agents can better learn about reward-causing state-action pairs which may not offer exogenous reward originally.
% % We first show that the expected reward at conditional states increases as a function of $n$.
% Suppose transitioning to $s_c$ is a general example of a reward-causing state-action pair.


% \begin{theorem}
% As $|T_i| \rightarrow \infty$, the expected team-based reward at a valuable conditional state $\mathbb{E} (TR_i(s_c))$ is strictly monotonically increasing.
% \label{thm:reward_distribution_max}
% \end{theorem}

% % \todo{note: $t = 0$ to require $s$ to be visited.}

% \begin{proof}
% We show that the maximum achievable reward at $s_c$ is monotonically increasing while the lower-bound is fixed.
% Assume at any timestep $t$ that agent $i$ is in state $s_c$ and all of $i$'s teammates are in $s_1$.
% This represents the scenario when $|T_i|$ can achieve the maximum possible reward at a single timestep, $\max(TR_i(s_c)) = \frac{r(|T_i|-1)}{|T_i|}$.
% The derivative of this is $\max(TR_i(s_c))' = \frac{r}{|T_i|^2}$.
% We know $\max(TR_i(s_c))' > 0$ since we assume $r > 0$ and $|T_i| \geq 1$; thus, we conclude that $\max(TR_i(s_c))$ is monotonically increasing as $|T_i| \rightarrow \infty$ and is upper-bounded by $r$ (i.e., $|T_i| - 1 < |T_i|$).
% Since $\min(TR_i(s_c)) = 0$ is fixed and the upper bound is converging to $r$, we conclude $\mathbb{E} (TR_i(s_c))$ is also monotonically increasing.
% \end{proof}


\begin{theorem}
The expected team-based reward $TR_{i[n]}$ when visiting $s_c$ monotonically increases as team size increases (i.e., $\mathbb{E} (TR_{i[X]}(s^t, a^t, s_c^{t+1})) \leq \mathbb{E} (TR_{i[Y]}(s^t, a^t, s_c^{t+1}))$ if $X \leq Y$).
\label{thm:reward_distribution_exp}
\end{theorem}


\begin{proof}
% Let $A$ and $B$ be two team sizes such that $A \leq B$.
Let $X' \equiv TR_{i[X]}(s^t, a^t, s_c^{t+1})$ and $Y' \equiv TR_{i[Y]}(s^t, a^t, s_c^{t+1})$ for two teams of size $X$ and $Y$ such that $X \leq Y$.
Suppose $C = Y' - X'$.
From the linearity of the expected value, we have:
\begin{equation}
    \mathbb{E}(C) = \mathbb{E} (Y' - X') = \mathbb{E}(Y') - \mathbb{E}(X').
    \label{eq:linearity_of_E}
\end{equation}
With the Non-negativity Property of the Expected Value Theorem, it holds that:

\[ C \geq 0 \Rightarrow \mathbb{E}(C) \geq 0. \]

Together with Equation~\ref{eq:linearity_of_E}, this yields $\mathbb{E}(Y') - \mathbb{E}(X') \geq 0$ if $Y \geq X$.
\end{proof}





% Theorem~\ref{thm:reward_distribution_exp} shows that the expected team-based reward for reward-causing state-action pairs (i.e., visiting $s_c$) increases as a function of team size, $n$.
Since agents seek to maximize the sum of future discounted rewards, Theorem~\ref{thm:reward_distribution_exp} places emphasis on the importance of their team's size for agents to learn about reward-causing state-action pairs.
It is important to note that no additional reward is generated for the expected value of visiting $s_c$ to increase.
Instead, rewards are shifted between agents in team $T_i$ that each have their own individual state-action experiences.
This is similar to reward redistribution in single-agent RL; however, rewards are redistributed among teammates instead of throughout an agent's memory.


Agents that receive the shifted rewards perceive certain state-action pairs to be more valuable than in settings without teams (if they yield no exogenous reward). % or with smaller teams.
% (i.e., these state-action pairs yield higher team-based reward in expectation).
As learning progresses, agents will ultimately become more attracted to these state-action pairs since they are now associated with some amount of reward.
As a result, a team would learn to divide labor and execute both reward-causing and exogenous-reward state-action pairs simultaneously.
This creates an inner-team autocurricula that provides feedback about the effectiveness of the team's joint policy (i.e., more efficiency leads to more overall reward and higher value for reward-causing state-action pairs).


% % \todo{Rethink this paragraph... dependent on team structure. In limit, I show they become equal in next section.}
% Dependent on an appropriate team structure, the expected value of reward-causing state action pairs, such as visiting $s_c$, will be greater than non-reward causing pairs that also provide no exogenous reward.
% % in specific team structures.
% This is because visiting $s_c$ would allow for more reward to be collected by the team in expectation, whereas visiting alternative states will not.

However, formalized in the next section, the ability for teams to identify and efficiently execute reward-causing state-action pairs is dependent on team structure.
Given a sub-optimal team structure, the reward signal may become diluted over the state space (i.e., if teams are too large).
Furthermore, while shifting rewards makes some state-action pairs more attractive, this reward is removed from other state-action pairs that actually do yield exogenous rewards.
Shifting too much reward away from these state-action pairs that do provide exogenous rewards has potential negative side-effects on what agents learn.

% While this helps agents identify valuable areas of the state space, we next show why team size should not simply be increased without consideration of the underlying environment.

% \begin{theorem}
% As $|T_i| \rightarrow \infty$, the expected team-based reward at a valuable conditional state converges to the mean exogenous reward any agent can achieve, $\mathbb{E} (TR_i(s_c)) \rightarrow \overline{R_i}$.
% \label{thm:reward_distribution_exp}
% \end{theorem}

% \begin{proof}
% % In Theorem~\ref{thm:reward_distribution_max}, we found that the highest reward possible for $T_i$ is $\max(TR_i(s)) = \frac{r(|T_i|-1)}{|T_i|}$ which is strictly monotonically increasing and bounded by $Z(s') = r$.
% By Theorem~\ref{thm:reward_distribution_max} we know that the maximum possible reward for $i$ at state $s_c$, $\max(TR_i(s_c))$, is monotonically increasing.
% The second derivative of this, $\max(TR_i(s_c))'' = - \frac{2r}{|T_i|^3}$, is negative; therefore, $\max(TR_i(s_c))$ increases more slowly as $|T_i| \rightarrow \infty$.
% % Since we know $\min(TR_i(s)) = 0$, we conclude $\mathbb{E} (TR_i(s))$ is also monotonically increasing, but bounded by $\mathbb{E} (TR_i)$.
% $TR_i$ is the combined reward of multiple agents with identical reward functions $R_i$, thus, the team-based reward function approximates a normal distribution centered about the mean exogenous reward for any agent $TR_i \approx \mathcal{N} (\overline{R_i}, \frac{\sigma^2_{R_i}}{\sqrt{|T_i|}})$ by the Central Limit Theorem.
% Since we know $\sigma^2_{R_i}$ is a constant and $|T_i| > 0$, the variance of $TR_i$ decreases, $\frac{\sigma^2_{R_i}}{\sqrt{|T|}} \rightarrow 0$, as $|T_i| \rightarrow \infty$, meaning $TR_i \rightarrow \overline{R_i}$.
% \end{proof}

% \begin{lemma}
% The team-based reward $TR_i^{|T_i|}$ converges to the mean of the reward function as team size increases, $TR_i^{|T_i|}(s^t, a^t, s_c)) \rightarrow \overline{R_i}$.
% \label{lem:reward_distribution_exp}
% \end{lemma}

% \begin{proof}
% Since the team-based reward is an aggregation of $|T_i|$ identical individual reward samples, let $TR_i^{|T_i|} \approx \mathcal{N} \left( \overline{R_i}, \frac{\sigma^2_{R_i}}{\sqrt{|T_i|}} \right)$ by the Central Limit Theorem.
% The derivative of the variance is $- \frac{\sigma_{R_i}}{ \sqrt{|T_i|^{3}}}$.
% Since $\sigma_{R_i}$ is constant and $|T_i| \geq 1$, the derivative is negative and the variance of $TR_i^{|T_i|} \rightarrow 0$ as a function of team size.
% \end{proof}

% Theorem~\ref{thm:reward_distribution_exp} suggests that the expected reward for $i$ at $s_c$ approaches $\overline{R_i}$ as team size grows.
% Taken together, these two theorems show how conditional reward states without exogenous reward are transformed to autonomously induce sub-goals, similar to in HRL or Options.
% Figure~\ref{fig:sub_goal} visualizes this process as a function of team size when the conditional exogenous reward received is $r = 1$ in our example environment.
% The $x$-axis shows different team sizes and the $y$-axis shows reward space.
% We see that both $\mathbb{E}(TR_i(s_c))$ and $\max(TR_i(s_c))$ are monotonically increasing and asymptotically approach 0.5 and 1, or $\overline{R_i}$ and $r$.


% \begin{figure}[t]
%     \centering
%     \includegraphics[width=\linewidth]{Figures/sub-goal.png}
%     \caption{How $\mathbb{E}(TR_i)$ and $\max(TR_i)$ change as a function of $|T_i|$ assuming the reward at $s_c$ is 0 and at $s_1$ is 1 if $s_c$ is visited, otherwise it is 0.}
%     \label{fig:sub_goal}
% \end{figure}


==> team_size.tex <==
\section{Impacts of Team Structure}
\label{sec:impacts}



In this section, we explore two dimensions of increasing team size and changing team structure: initial positives of increasing team size and inevitable negatives of teams that are too big.
We propose that there exists an equilibrium between these two with high performance.

For the remainder of the paper, consider the existence of two states: $s$ and $s'$.
Reward in SGs is conditioned on the environment and other agents; thus, consider a scenario that state $s$ offers no explicit reward; however, environmental reward is given at $s'$ \emph{conditioned} on $s$.
This means the importance of visiting $s$ must be learned for any reward to be obtained at $s'$.

\input{increase_reward_distribution}
\input{decrease_state_information}
